The Impact of Qubit Connectivity on Quantum Advantage in Noisy IQP Circuits

Instantaneous Quantum Polynomial-time (IQP) circuits are a candidate for demonstrating near-term quantum advantage, as their sampling task is believed to be classically hard in the ideal theoretical setting under standard complexity-theoretic assumptions. In noisy implementations, however, this hardness can disappear once circuit depth exceeds a noise-dependent critical threshold. We show that qubit connectivity is a key parameter in this transition, since sparse architectures require additional routing to implement long-range interactions, thereby increasing compiled circuit depth. To make this explicit, we present a connectivity-aware analysis of compiled IQP circuits. For a fixed abstract IQP instance, different hardware connectivity graphs yield different compiled depths and thus different effective positions relative to the noisy-IQP simulatability boundary. We quantify this architecture-dependent shift using the compiled depth overhead and the corresponding simulatability margin. We combine analytic depth estimates for sparse geometries, including the two-dimensional grid, with native-gateset-aware compilation experiments across seven hardware-grounded experimental device models derived from publicly available topologies. To compare these device models under a unified empirical framework, we approximate the effective noise level primarily through reported two-qubit gate error rates. This lets us compare how much effective noise sparse and fully connected architectures can tolerate for the same position relative to the noisy-IQP simulatability boundary. Our results show that sparse connectivity requires a lower effective noise level to sustain the same margin relative to the noisy-IQP simulatability boundary, and they provide a quantitative framework for determining when compiled IQP experiments are likely to remain outside, or instead enter, the classically simulatable regime.

==> forJournal/draftnarrative.tex <==
\leo{We ideally want to have a more complete understanding of noise impact for the later stage journal}

\section{Methods}
\subsection{Connectivity-induced simulatability shift}
\label{sec:ciss}
We formalize how hardware connectivity changes the effective position of an IQP implementation relative to the known noisy-IQP simulatability boundary by explicitly separating a logical circuit family from its compiled physical realizations.

Throughout this section, $D$ denotes a scheduled two-qubit entangling depth (in layers), and $p$ denotes an abstract effective noise strength as it appears in noisy-IQP simulatability theory. We will later instantiate these abstract quantities with compilation-dependent values $(D_H,p_{\mathrm{eff}}(H))$ computed from the compiled circuit and calibration data.

We distinguish from the outset two complementary, exposure-based perspectives on connectivity-induced degradation.
First, a \emph{global depth–noise exposure} framework which tracks how compilation moves an instance in the $(D,p)$ plane relative to the critical-depth boundary $D_\ast(p,k)$ established in noisy-IQP analyses \cite{Bremner_2017}. This viewpoint treats noise as effectively homogeneous and summarizes compilation effects through the pair $(D_H, p_{\mathrm{eff}}(H))$, leading to the depth-based simulatability margin $m(H)$ defined as a signed distance to the proven global threshold and to the associated global exposure score $\chi_H := p_{\mathrm{eff}}(H)\,D_H$ introduced in Sec.~\ref{sub:correlation_decay}.
Second, a \emph{support-resolved correlator exposure} framework which tracks how routing and idling attenuate specific multi-qubit $X$-correlators associated with individual interaction supports. Classical simulability mechanisms for noisy IQP circuits ultimately rely on the suppression of high-weight Pauli correlations and the breakdown of anticoncentration \cite{Bremner_2017, Napp_2022, Bravyi2022}. Connectivity-induced routing can concentrate noise exposure on particular supports, exponentially damping the corresponding correlators even when the global depth remains below $D_\ast(p,k)$. This viewpoint leads to the worst-support decay score $\zeta_H$ and the associated structure-aware margin $m_\zeta(H)$, defined as a signed distance to a correlator-decay threshold $\tau_\zeta$ that marks when a support’s $X$-correlator is treated as effectively negligible (e.g.\ below a chosen approximation or measurement-noise scale); in contrast to $m(H)$, which is directly anchored in the noisy-IQP theorem, $(\zeta_H,m_\zeta(H))$ provide a physically motivated but not theorem-derived diagnostic for support-level degradation.

We now formalize the global phase-diagram perspective before turning to the structure-aware analysis. In particular, we first define the logical circuit family, its compiled depth under different connectivity graphs, and the resulting global simulatability margin $m(H)$.

Let $C$ denote an $n$-qubit $k$-local IQP circuit instance specified by a set of commuting Pauli strings $\{X_s: 1\le |s|\le k\}$ with angles $\{\theta_s\}$ (cf. Eq.~\eqref{eq:iqp_unitary}). The circuit induces an interaction hypergraph $G_C$ over $[n]$, where each $k'$-body term $(k'\le k)$ corresponds to a hyperedge on the participating qubits.

We define the ideal logical depth $D_{\mathrm{ideal}}$ as the scheduled depth
(in layers of native two-qubit entangling gates) required to implement $C$
assuming an all-to-all hardware graph, i.e., any pair of qubits can be acted on
directly without routing (SWAP insertion). Importantly, this assumption concerns
only qubit connectivity: each $k$-local term in Eq.~\eqref{eq:iqp_unitary} is
still synthesized using the same fixed native gate set (single- and two-qubit
gates) as in the hardware-constrained setting.

Let $H$ denote a hardware connectivity graph on the same $n$ qubits (or on $N\ge n$ physical qubits with an injection map, which we suppress for clarity). We consider three representative connectivity classes:
\begin{itemize}
    \item $H_{\mathrm{2D}}$: a bounded-degree 2D lattice (or heavy-hex-like sparse graph);
    \item $H_{\mathrm{IBM}}$: a device-specific superconducting connectivity graph;
    \item $H_{\mathrm{FC}}$: an (approximately) fully connected graph (ion-trap- or neutral atom like).
\end{itemize}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.3\textwidth]{paper_images/topologies/topology_comparison.png}
    \caption{Connectivity topologies of current quantum hardware platforms (12 qubits). 
    \textbf{Top-left}: Fully connected (ideal)---any qubit can interact with any other directly. 
    \textbf{Top-right}: Google Sycamore uses a 2D grid. 
    \textbf{Bottom-left}: IBM heavy-hex has degree-2 and degree-3 nodes. 
    \textbf{Bottom-right}: Rigetti Aspen employs octagonal units.
    Sparse topologies require SWAP gates to route interactions between non-adjacent qubits, 
    increasing circuit depth.}
    \label{fig:topologies}
\end{figure}

Given a hardware graph $H$, compilation produces a physical circuit
$\widetilde{C}_H := \mathrm{Compile}(C;H)$,
which implements the same logical unitary (up to permissible rewrites) using the native gate set and routing operations (e.g., SWAP networks) required by $H$. We denote by $D_H$ the resulting physical scheduled depth of $\widetilde{C}_H$ in units of entangling-gate layers (or, more generally, in units consistent with the noise insertion points used in Sec.~\ref{sec:ptsiqp}).

The connectivity-induced depth overhead is then
\begin{equation}
    \Delta D(H) \;:=\; D_H - D_{\mathrm{ideal}} \;\ge\; 0.
\end{equation}
By construction, we expect
\begin{equation}
\Delta D(H_{\mathrm{FC}})\;\le\;\Delta D(H_{\mathrm{IBM}}),\ \Delta D(H_{\mathrm{2D}}),
\end{equation}
since full connectivity minimizes (and often eliminates) routing overhead for nonlocal interactions.

The noisy-IQP result reviewed in Sec.~\ref{sec:ptsiqp} provides a noise-dependent critical depth scale $d_\ast(p,k)$ such that circuits exceeding this scale fall into an efficiently classically simulatable regime (up to the theorem’s approximation guarantees). We therefore interpret $\Delta D(H)$ as shifting the implemented circuit along the ``depth axis'' toward simulatability.

To make this quantitative in the global phase-diagram picture, we define a simulatability margin under hardware $H$ as
\begin{equation}
m(H) \;:=\; D_\ast\!\bigl(p_{\mathrm{eff}}(H),k\bigr) \;-\; D_H,
\end{equation}
where $p_{\mathrm{eff}}(H)$ is an effective per-layer noise parameter for the compiled circuit $\widetilde{C}_H$. For $D_\ast\!\bigl(p_{\mathrm{eff}}(H),k\bigr)$ see~\eqref{eq:critical_depth}. Positive margin $m(H)>0$ indicates the implementation remains on the ``non-certified'' side of the known simulatability condition, whereas negative margin $m(H)<0$ indicates the implementation is predicted to lie in the simulatable regime.

The quantity $m(H)$ therefore captures a \emph{global} constraint: it depends only on the compiled depth $D_H$ and the effective noise strength $p_{\mathrm{eff}}(H)$, and ignores how noise is distributed across different logical supports. In particular, it does not distinguish whether routing overhead is uniformly spread or concentrated on specific multi-qubit interactions.

Finally, we define the connectivity-induced simulatability shift relative to the idealized schedule as
\begin{equation}
S(H) \;:=\; \bigl(D_{\mathrm{ideal}},p_{\mathrm{ideal}}\bigr)\ \mapsto\ \bigl(D_H, p_{\mathrm{eff}}(H)\bigr),    
\end{equation}
i.e., the architecture-dependent map from a logical instance to its effective operating point in the $(p,D)$ phase diagram. In our setting, the primary effect is a upward shift in depth by $\Delta D(H)$ (and typically a rightward shift in effective noise as well), with $H_{\mathrm{FC}}$ producing the smallest shift among the considered architectures.

The complementary structure-aware quantities $(\zeta_H,m_\zeta(H))$ are defined in Sec.~\ref{sub:correlation_decay} and used later to combine global and worst-support constraints.

The remainder of this section first quantifies the global depth inflation (including analytic estimates for $D_H$ on sparse geometries), and then introduces the structure-aware correlator decay framework. The two perspectives are finally combined into a unified architecture-level indicator $\mathcal{I}_H$ that \textcolor{red}{summarizes both global and worst-support degradation mechanisms in a single score, without claiming a sharp or necessary boundary.}\textcolor{green}{(Softens the language about $\mathcal{I}_H$ so it is clearly described as a summary indicator, not as a proven hardness boundary.)} \leo{my goal right now is to get a better simulability boundary sinze the zeta is just speculativekly tied to simulability.}
We next quantify $D_H$ analytically for a representative sparse geometry (a 2D grid), which will later be used to evaluate the global margin $m(H)$ and the implied noise-budget ratios.
\cy{We will also need to plot the phase diagram and plot arrows as compilation shifts on that}

\subsection{Theoretical Estimation of $D_H$ on a 2D Grid}
\label{sec:theory_DH_2D}

In this subsection we provide a theoretical (order-wise) estimate of the compiled
two-qubit entangling depth $D_H$ when mapping an $n$-qubit IQP instance to a
2D nearest-neighbor grid graph $H_{\mathrm{2D}}$ (e.g., an $\sqrt{n}\times\sqrt{n}$
lattice). The purpose is not to predict compiler-optimal constants, but to
quantify how limited connectivity induces an \emph{upward} shift in depth, and
thus reduces the simulatability margin via the critical-depth criterion in
Eq.~\eqref{eq:critical_depth}.

\paragraph{Setup.}
We assume a fixed native gate set with arbitrary one-qubit gates and a native
two-qubit entangling gate between adjacent vertices of $H_{\mathrm{2D}}$. We
measure depth in \emph{two-qubit entangling layers}. Let $C$ denote an ideal IQP
circuit instance, and let $D_{\mathrm{ideal}}$ be its two-qubit depth under
complete connectivity (no routing SWAPs), as defined in Sec.~\ref{sec:ciss}.
Compiling $C$ to the 2D grid produces a physical circuit
$\widetilde{C}_{\mathrm{2D}}$ with depth $D_{\mathrm{2D}}:=D_{H_{\mathrm{2D}}}$
and overhead $\Delta D(H_{\mathrm{2D}})=D_{\mathrm{2D}}-D_{\mathrm{ideal}}$.

We write $\mathrm{dist}_{\mathrm{2D}}(u,v)$ for the graph distance (Manhattan
distance) between two qubits $u,v$ on the grid.

\subsubsection*{(1) Random-pair interaction demand: distance-based lower bound}

A convenient abstraction is to view each two-qubit entangling operation in the
chosen 1q/2q decomposition of $C$ as a demand to apply an entangling gate on a
pair $(u,v)$. If $(u,v)$ is not an edge of $H_{\mathrm{2D}}$, routing is required
to bring the two qubits adjacent.

A simple (but general) distance-based lower bound follows from the fact that
each SWAP can reduce the distance between a target pair by at most $1$:
implementing a two-qubit gate on $(u,v)$ requires at least
$\mathrm{dist}_{\mathrm{2D}}(u,v)-1$ adjacency-creating moves.\footnote{Depending
on the routing model, the constant prefactor can vary (e.g., whether both qubits
move), but the scaling in $\mathrm{dist}$ is unavoidable.} Summing over all
two-qubit entangling operations yields a coarse lower bound on routing cost and
hence on depth:
\begin{equation}
D_{\mathrm{2D}}
\;\gtrsim\;
D_{\mathrm{ideal}}
\;+\;
\frac{1}{\Lambda}\sum_{(u,v)\in \mathcal{E}}
\bigl(\mathrm{dist}_{\mathrm{2D}}(u,v)-1\bigr),
\label{eq:DH_2D_dist_lower}
\end{equation}
where $\mathcal{E}$ is the multiset of two-qubit interaction pairs induced by
the chosen decomposition of $C$, and $\Lambda$ is the maximum number of
distance-reducing SWAP ``moves'' that can be executed in parallel per layer
(on a grid, $\Lambda=\Theta(n)$ in the best case).\footnote{Eq.~\eqref{eq:DH_2D_dist_lower}
is intentionally stated as an order-wise bound: it formalizes that large typical
distances force nontrivial depth overhead even under aggressive parallel
routing.}

For interaction demands that are effectively \emph{random} over pairs, which is
a reasonable proxy when the IQP instance induces near-complete mixing over
qubit pairs after decomposition, the typical grid distance satisfies
$\mathbb{E}[\mathrm{dist}_{\mathrm{2D}}(u,v)]=\Theta(\sqrt{n})$ for uniformly
random $u,v$ \citemark. Consequently, the average per-gate routing requirement
scales as $\Theta(\sqrt{n})$, implying a multiplicative depth overhead that can
grow with $\sqrt{n}$ if many long-range pairs must be realized.

\subsubsection*{(2) Exploiting $k$-local structure: support diameter lower bound}

We now leverage the fact that IQP circuits are $k$-local in the sense of
Eq.~\eqref{eq:iqp_unitary}: each generator term $\exp(i\theta_s X_s)$ involves
only $|s|\le k$ qubits. Under a standard 1q/2q synthesis, each $k'$-body term
($k'\le k$) can be implemented using $O(k')$ two-qubit entangling gates, e.g.,
by computing parities onto one qubit in $s$ (CNOT tree), applying a one-qubit
phase rotation, and uncomputing. Thus, for constant $k$, each term expands to
$O(k)$ two-qubit gates, and the routing overhead is governed by the geometry of
the participating qubits on the grid.

Let $\mathrm{diam}_{\mathrm{2D}}(s):=\max_{u,v\in s}\mathrm{dist}_{\mathrm{2D}}(u,v)$
denote the diameter of the subset $s$ under the grid metric. Any 2D
implementation of a multi-qubit interaction supported on $s$ must communicate
information across this diameter, which induces a depth cost at least linear in
$\mathrm{diam}_{\mathrm{2D}}(s)$. In particular, there exists a constant $c>0$
such that the two-qubit depth required to realize a single $k'$-local term
obeys
\begin{equation}
D_{\mathrm{2D}}(s)
\;\ge\;
c\,\mathrm{diam}_{\mathrm{2D}}(s),
\label{eq:term_depth_lower}
\end{equation}
up to additive $O(1)$ terms that depend only on the synthesis approach.
Therefore, for an IQP instance with term set $\mathcal{S}$ and a layer
partition $\{\mathcal{S}_t\}_{t=1}^{D_{\mathrm{ideal}}}$ under complete
connectivity, a conservative lower bound is
\begin{equation}
D_{\mathrm{2D}}
\;\gtrsim\;
\sum_{t=1}^{D_{\mathrm{ideal}}}
\max_{s\in \mathcal{S}_t}\mathrm{diam}_{\mathrm{2D}}(s).
\label{eq:DH_2D_klocal_lower}
\end{equation}
For random $k$-tuples $s$ placed on an $\sqrt{n}\times\sqrt{n}$ grid,
$\mathbb{E}[\mathrm{diam}_{\mathrm{2D}}(s)]=\Theta(\sqrt{n})$ even for constant
$k\ge 2$, so Eq.~\eqref{eq:DH_2D_klocal_lower} again predicts a nontrivial upward
depth shift unless placement restricts the supports $s$ to be geometrically
local.

\paragraph{Constructive upper bound (order-wise).}
Conversely, standard 2D routing results imply that arbitrary qubit permutations
can be implemented in $O(\sqrt{n})$ SWAP depth on a 2D grid. As a consequence, an
arbitrary complete-graph two-qubit layer (a matching) can be realized with an
$O(\sqrt{n})$ depth overhead in the worst case by (i) routing qubits to make the
desired pairs adjacent, (ii) applying all entangling gates in parallel, and
(iii) optionally routing back. Therefore, for circuits whose ideal schedule
consists of $D_{\mathrm{ideal}}$ two-qubit layers, we obtain the order-wise
upper bound
\begin{equation}
D_{\mathrm{2D}}
\;\lesssim\;
O(\sqrt{n})\cdot D_{\mathrm{ideal}},
\label{eq:DH_2D_upper}
\end{equation}
with constants depending on the routing scheme and whether restoration to the
original layout is required.

\paragraph{Implication for the simulatability margin on a 2D grid}
Combining the depth estimate above with the effective-noise aggregation model in
Sec.~\ref{sec:ptsiqp} yields an estimated operating point
$(p_{\mathrm{eff}}(H_{\mathrm{2D}}),D_{\mathrm{2D}})$. We define the (bound-based)
simulatability margin on the 2D grid as
\begin{equation}
m_{\mathrm{2D}}
\;:=\;
D_\ast\!\bigl(p_{\mathrm{eff}}(H_{\mathrm{2D}}),k\bigr)
\;-\;
D_{\mathrm{2D}},
\label{eq:margin_2D}
\end{equation}
where $D_\ast(p,k)$ follows the critical-depth scaling in Eq.~\eqref{eq:critical_depth}.
Using the upper bound in Eq.~\eqref{eq:DH_2D_upper} gives a conservative
sufficient condition for entering the simulatable regime:
\begin{equation}
O(\sqrt{n})\cdot D_{\mathrm{ideal}}
\;\gtrsim\;
D_\ast\!\bigl(p_{\mathrm{eff}}(H_{\mathrm{2D}}),k\bigr),
\label{eq:2D_sufficient_simulable}
\end{equation}
whereas the lower bounds in Eqs.~\eqref{eq:DH_2D_dist_lower}
and~\eqref{eq:DH_2D_klocal_lower} quantify when nonlocal interaction supports
necessarily induce a large upward shift in depth.

Because the simulatability theory defines $p$ for an abstract interleaved Pauli
channel, we do not interpret $p$ as a directly measured hardware gate error
rate. Instead, we use the phase boundary as a \emph{noise-budget constraint}:
for a compiled depth $D_H$.
Let $p_{\mathrm{req}}(D_H,k)$ denote the maximal noise strength such that the
simulatability condition $D_H \le D_\ast(p,k)$ is still satisfied, i.e.,
\[
p_{\mathrm{req}}(D,k) := \sup\{p: D \le D_\ast(p,k)\}.
\]
For two architectures with depths $D_{\mathrm{FC}}$ (fully connected) and
$D_{\mathrm{S}}=D_{\mathrm{FC}}+\Delta D$ (sparse), monotonicity of $D_\ast$ in
$p$ implies $p_{\mathrm{req}}(D_{\mathrm{S}},k) \le p_{\mathrm{req}}(D_{\mathrm{FC}},k)$.
Moreover, using the scaling $D_\ast(p,k)=\Theta\!\bigl(p^{-1}\log(k/p)\bigr)$
yields the first-order ratio estimate
\begin{equation}
\frac{p_{\mathrm{req}}(D_{\mathrm{S}},k)}{p_{\mathrm{req}}(D_{\mathrm{FC}},k)}
\;=\;
O\!\left(\frac{D_{\mathrm{FC}}}{D_{\mathrm{S}}}\right)
\;=\;
O\!\left(\frac{D_{\mathrm{FC}}}{D_{\mathrm{FC}}+\Delta D}\right),
\label{eq:noise_budget_ratio}
\end{equation}
where the $O(\cdot)$ hides constant factors and the weakly varying logarithmic
correction induced by $\log(k/p)$, which changes slowly over the operating
regime of interest. Consequently, non–fully connected architectures must achieve proportionally lower effective noise to compensate for routing-induced depth inflation,
whereas fully connected architectures can tolerate higher noise (or larger
instances) while maintaining the same simulatability margin. \cy{We can actually use different setting and plot how low the spare/non fully connected hardware should be to have the same simulatability regime as fully connected.}
\leo{FROM HERE THE PAPER MIGHT BE CUT - this second analysis might be part of a Journal version. The team also is pushing towards executing experiments on real hardware.
----------------------}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Structure-aware correlation decay and worst-support noise exposure}
\label{sub:correlation_decay}

Beyond the global depth-based comparison of
Eq.~\eqref{eq:noise_budget_ratio}, we refine the
architecture–noise tradeoff by introducing a
\emph{structure-aware correlation-decay score}.
For each $k$-local IQP interaction
$U_j=\exp(i\theta_j X_{S_j})$ acting on a support
$S_j\subseteq[n]$, the compiled circuit $\widetilde{C}_H$
induces both gate-dependent noise and idle-time dephasing
on the qubits in $S_j$.
While the global analysis is governed by a single scalar depth $D_H$. In contrast, the structure-aware analysis replaces $D_H$ by a collection of support-specific depths $\{d_{S_j}\}_j$, since different interaction supports can experience very different routing and idling exposure.
To quantify the resulting loss of $X$-basis coherence,
we assign to each interaction an \emph{effective interaction depth}
\begin{equation}
d_{S_j}
:= D^{(2q)}_{S_j} + \eta\, D^{(\mathrm{idle})}_{S_j},
\label{eq:dsj}
\end{equation}
where $D^{(2q)}_{S_j}$ counts the scheduled two-qubit
layers \leo{ideally term would be diagonal gates from \cite{rajakumar2025polynomial}} touching any qubit in $S_j$,
$D^{(\mathrm{idle})}_{S_j}$ counts the corresponding idle
layers, and $\eta\in[0,1]$ weights idle dephasing relative
to two-qubit gate noise using calibrated gate durations
and $T_2$ data.

The effective error probability accumulated on $S_j$ is
\begin{equation}
p_{S_j}
:= 1 -
\Bigg[ \prod_{g\in\mathcal{G}(S_j)} (1-\epsilon_g)\Bigg]
\Bigg[ \prod_{q\in S_j}
e^{-t^{(\mathrm{idle})}_q/T_{2,q}} \Bigg],
\label{eq:psj}
\end{equation}
where $\mathcal{G}(S_j)$ denotes the set of physical gates
whose support intersects $S_j$,
$\epsilon_g$ is the calibrated error-per-gate (including
SWAP decompositions),
and $t^{(\mathrm{idle})}_q$ is the total idle time of qubit $q$
during the implementation window of $U_j$.
Here $p_{S_j}$ is a \emph{support- and window-specific} accumulated error probability, whereas $p_{\mathrm{eff}}(H)$ is a \emph{global effective} noise strength used to instantiate the abstract parameter $p$ in the critical-depth bound $D_\ast(p,k)$.

We define the interaction-specific
\emph{correlation-decay exponent}
\begin{equation}
\Lambda_j := p_{S_j}\, d_{S_j},
\label{eq:lambdaj}
\end{equation}
provides an approximate bound on\textcolor{green}{(Softens the claim: “upper-bounds” → “provides an approximate bound on”, to reflect the heuristic nature.)} the attenuation of the Pauli-$X$
correlator on $S_j$ via
\begin{equation}
\langle X_{S_j}\rangle_{\mathrm{noisy}}
\approx
\langle X_{S_j}\rangle_{\mathrm{ideal}}
e^{-\Lambda_j}.
\label{eq:correlator_decay}
\end{equation}

The \emph{correlation-decay score} of hardware $H$ is
\begin{equation}
\zeta_H := \max_j \Lambda_j,
\label{eq:zetaH}
\end{equation}
capturing the worst-case multi-qubit coherence loss
across all IQP interactions.
Unlike the global exposure measure in
Eq.~\eqref{eq:noise_budget_ratio},
$\zeta_H$ resolves support-dependent variations
arising from routing geometry and idle exposure and is intended as a structure-aware indicator of when specific high-weight supports have been strongly damped.
\leo{this tau is too arbitrary}
To place $\zeta_H$ on the same \textit{distance-to-threshold } footing as the global margin $m(H)$, we define the per-support structure-aware margin
\begin{equation}
m_\zeta^{(S_j)}(H) := \tau_\zeta - \Lambda_j,
\end{equation}
and the worst-support (architecture-level) structure-aware margin
\begin{equation}
m_\zeta(H) := \min_j m_\zeta^{(S_j)}(H)
= \tau_\zeta - \zeta_H.
\label{eq:mzeta}
\end{equation}
Here $\tau_\zeta>0$ is a phenomenological threshold that sets the scale at which a support’s $X$-correlator is regarded as effectively negligible, for example because its contribution falls below a chosen approximation error or below the experimental noise floor. We do not derive $\tau_\zeta$ from a simulability theorem; instead, it plays the role of a tunable accuracy parameter in the structure-aware diagnostic. \textcolor{red}{Positive $m_\zeta(H)$ indicates that all interaction supports remain below the chosen correlator-decay threshold, whereas negative $m_\zeta(H)$ indicates that at least one support has accumulated enough noise–depth exposure for its $X$-correlator to be treated as effectively collapsed at that threshold.}

\subsubsection{Inverting the structure-aware constraint}

Imposing the working condition that all supports remain below the chosen decay threshold, i.e.\ $\zeta_H \le \tau_\zeta$, yields, for each interaction,
\begin{equation}
p_{\mathrm{req}}^{(S_j)}(d_{S_j})
=
\frac{\tau_\zeta}{d_{S_j}},
\label{eq:preq_sj}
\end{equation}
so that the architecture-level requirement is governed by
the most restrictive support,
\begin{equation}
p_{\mathrm{req}}^{(\zeta)}(H)
=
\frac{\tau_\zeta}{d_{\max}(H)},
\qquad
d_{\max}(H) := \max_j d_{S_j}.
\label{eq:preq_zeta}
\end{equation}
The quantity $p_{\mathrm{req}}^{(\zeta)}(H)$ therefore specifies, for a given choice of $\tau_\zeta$, how small the effective noise must be for the worst-exposed support to stay above the correlator threshold used in our diagnostic.

Let $d_{\max}^{FC}$ and $d_{\max}^{S}$ denote the maximal
interaction-specific depths under full connectivity
and under a sparse hardware graph, respectively.
Monotonicity of $p_{\mathrm{req}}^{(\zeta)}$
in $d_{\max}$ gives the structure-aware ratio
\begin{equation}
\frac{
p_{\mathrm{req}}^{(\zeta)}(S)
}{
p_{\mathrm{req}}^{(\zeta)}(FC)
}
=
\frac{d_{\max}^{FC}}{d_{\max}^{S}}
=
O\!\left(
\frac{d_{\max}^{FC}}
     {d_{\max}^{FC} + \Delta d_{\max}}
\right),
\label{eq:local_ratio}
\end{equation}
where $\Delta d_{\max}
:= d_{\max}^{S}-d_{\max}^{FC}$
encodes the architecture-induced amplification
of worst-support exposure.

\subsubsection{Global and structure-aware combination}

In addition to $\zeta_H$,
define the global exposure score
\begin{equation}
\chi_H := p_{\mathrm{eff}}(H)\, D_H,
\label{eq:chiH}
\end{equation}
i.e., we take $d_{\mathrm{eff}}(H):=D_H$ so that the global exposure uses the same compiled two-qubit depth as in Sec.~\ref{sec:ciss}. \textcolor{red}{Analogously to $\tau_\zeta$, we introduce a global exposure threshold $\tau_\chi>0$ that sets the scale at which the product $p_{\mathrm{eff}}(H)D_H$ is regarded as large enough for the noisy-IQP depth bound to be relevant at the chosen accuracy.}\textcolor{green}{(Introduces $\tau_\chi$ in the same spirit as $\tau_\zeta$ and ties it to accuracy.)}
Combining the global noise requirement
$p_{\mathrm{req}}(D_H,k)$ (as defined above)
with Eq.~\eqref{eq:preq_zeta},
the allowable architecture-level noise is
\begin{equation}
p_{\mathrm{req}}^{(\mathrm{comb})}(H)
:=
\min\!\Bigl\{
p_{\mathrm{req}}(D_H,k),
\;
p_{\mathrm{req}}^{(\zeta)}(H)
\Bigr\}.
\label{eq:preq_combined}
\end{equation}

We then define a unified architecture-level simulability indicator\leo{but is it an indicator? I want an indicator but we might have to drop this narrative and just develop the correlation exposure through an example.}
\begin{equation}
\mathcal{I}_H
:=
\max\!\left\{
\frac{p_{\mathrm{eff}}(H)}
     {p_{\mathrm{req}}(D_H,k)},
\;
\frac{p_{\mathrm{eff}}(H)}
     {p_{\mathrm{req}}^{(\zeta)}(H)}
\right\}
\approx
\max\!\left\{
\frac{\chi_H}{\tau_\chi},
\;
\frac{\zeta_H}{\tau_\zeta}
\right\}.
\label{eq:hardness_indicator}
\end{equation}
The approximation uses the first-order inversion $p_{\mathrm{req}}(D,k)\propto 1/D$ implied by the scaling of $D_\ast(p,k)$, up to slowly varying logarithmic factors. We interpret $\mathcal{I}_H\lesssim 1$ as an operating point where neither the global depth-based mechanism nor the worst-support decay mechanism is predicted (for the chosen thresholds) to be strongly active, and $\mathcal{I}_H\gtrsim 1$ as a regime where at least one of the two sufficient degradation mechanisms is expected to substantially suppress the IQP correlations. We do not claim $\mathcal{I}_H$ to define a sharp or necessary boundary between hard and easy regimes; rather, it aggregates two complementary sufficient diagnostics into a single architecture-dependent score.\textcolor{green}{(Clarifies how to interpret $\mathcal{I}_H$, explicitly calls the mechanisms “sufficient degradation mechanisms”, and states that $\mathcal{I}_H$ is not a sharp or necessary hardness boundary.)}

Finally, combining the global depth ratio
of Eq.~\eqref{eq:noise_budget_ratio}
with Eq.~\eqref{eq:local_ratio}
yields the mixed architecture penalty
\begin{equation}
\frac{
p_{\mathrm{req}}^{(\mathrm{comb})}(S)
}{
p_{\mathrm{req}}^{(\mathrm{comb})}(FC)
}
\;\le\;
\min\!\left\{
O\!\left(\frac{D_{FC}}{D_S}\right),
\;
O\!\left(\frac{d_{\max}^{FC}}{d_{\max}^{S}}\right)
\right\}.
\label{eq:combined_ratio}
\end{equation}
Sparse-connectivity hardware therefore suffers
two distinct penalties:
global depth inflation and worst-support
correlation decay.


%TENTATIVE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\textcolor{red}{
\paragraph{Tentative structural refinement of the simulability indicator}
The correlator-based score $\zeta_H$ quantifies when particular supports $S_j$ are strongly noise-damped, but it does not, by itself, certify classical simulability. A structural refinement arises by analysing the interaction pattern that remains once high-exposure supports (those with $\Lambda_j \ge \tau_\zeta$) are pruned.
Let $G_{\mathrm{eff}}(H)$ denote the effective interaction hypergraph after removing all such supports. Let $\{C_\ell\}$ be its connected components, and define}
\[
F_H := \max_\ell |C_\ell|.
\]
\textcolor{red}{Next, obtain $G_{\mathrm{eff}}^{\mathrm{clique}}(H)$ by replacing each hyperedge with a clique on its qubits, and define its treewidth}
\[
\mathrm{tw}_H := \mathrm{tw}\!\bigl(G_{\mathrm{eff}}^{\mathrm{clique}}(H)\bigr).
\]

\textcolor{red}{
\emph{Component-size branch.}
Because the pruned effective model has no cross-component interactions, its output distribution factorizes as}
\[
P_H(x_1,\dots,x_n)
=
\prod_\ell P_{H,\ell}(x_{C_\ell}).
\]
\textcolor{red}{
Exact simulation of each component $C_\ell$ costs at most $2^{O(|C_\ell|)}$, so}
\[
T_{\mathrm{fact}}(H)
\;\le\;
\sum_\ell 2^{O(|C_\ell|)}
\;\le\;
n\cdot 2^{O(F_H)}.
\]
\leo{Picking c will be something to think about for experiments}
\textcolor{red}{
If $F_H \le c\log n$, then $2^{O(F_H)} = n^{O(1)}$ and thus $T_{\mathrm{fact}}(H)$ is polynomial in $n$. If $F_H = O((\log n)^2)$, the runtime becomes $n^{O(\log n)}$ (quasi-polynomial). This provides a sufficient structural condition for efficient classical simulation once correlator-pruned interactions have disconnected the model into logarithmic-sized components.}

\textcolor{red}{
\emph{Treewidth branch.}
Exact simulation can also proceed via tensor-network contraction on $G_{\mathrm{eff}}^{\mathrm{clique}}(H)$. Standard junction-tree bounds give}
\[
T_{\mathrm{TN}}(H)
=
\mathrm{poly}(n)\,2^{O(\mathrm{tw}_H)}.
\]
\textcolor{red}{
Hence $\mathrm{tw}_H \le c\log n$ implies $T_{\mathrm{TN}}(H)=\mathrm{poly}(n)$, and $\mathrm{tw}_H = O((\log n)^2)$ implies quasi-polynomial runtime.}

\textcolor{red}{
\emph{Structural certificate.}
Define}
\[
\Phi_H := \max\{F_H,\ \mathrm{tw}_H\}.
\]
\textcolor{red}{
If $\Phi_H = O(\log n)$ then the pruned model admits polynomial-time classical simulation. Thus, once noise pushes enough supports above $\tau_\zeta$ so that the surviving interaction structure satisfies $F_H,\mathrm{tw}_H = O(\log n)$, the instance becomes classically simulatable by well-understood classical algorithms, independently of the global depth-based criterion.}

\leo{its a mess to put red but this also tentative}
\paragraph{Certified simulable condition (tentative)}
We separate two sufficient branches for classical simulability:
(i) a global noisy-IQP branch controlled by the depth/noise exposure, and
(ii) a correlator+structure branch where heavily exposed supports are pruned and the residual interaction structure is classically easy.

Define the global exposure indicator
\[
I_{\mathrm{glob}}(H)
:=
\frac{\chi_H}{\tau_\chi},
\]
and the correlator+structure indicator
\[
I_{\mathrm{corr+str}}(H)
:=
\min\!\left\{
\frac{\zeta_H}{\tau_\zeta},
\,
\frac{c \log n}{\Phi_H}
\right\},
\]
where $c>0$ is a universal constant and
$\Phi_H := \max\{F_H,\mathrm{tw}_H\}$ as above.
The architecture-level simulability indicator is then
\[
\mathcal{I}_H
:=
\max\!\left\{
I_{\mathrm{glob}}(H),
\,
I_{\mathrm{corr+str}}(H)
\right\}.
\]
We say that an implementation is \emph{certified simulable} whenever
\[
\mathcal{I}_H \;\ge\; 1.
\]
In this formulation, $\zeta_H$ never certifies simulability by itself:
the correlator-based branch requires simultaneously
(a) that some supports have accumulated enough exposure to be pruned
($\zeta_H \ge \tau_\zeta$),
and
(b) that the pruned interaction structure is logarithmic in component size
and/or treewidth ($\Phi_H \le c \log n$),
which guarantees a known polynomial-time classical simulation of the effective model.
The global branch $I_{\mathrm{glob}}(H) \ge 1$ corresponds instead to crossing
the noisy-IQP depth/noise threshold via $\chi_H$.

==> forJournal/previous_intro.tex <==
We frame this as a shift in the simulatability phase diagram: for a fixed logical IQP circuit family, different hardware graphs yield different compiled depths and different effective noise parameters, thereby moving the physical experiment along the axis controlling known simulatability thresholds. Our analysis proceeds in three main steps:
\begin{enumerate}
    \item \textbf{Logical IQP families.} We specify representative IQP circuit families and define the associated interaction patterns.
    \item \textbf{Compilation under hardware graphs.} For each hardware connectivity graph $H$, we compile the same logical circuits into physical circuits $\tilde C_H$, measuring routing overhead through added SWAPs, added two-qubit depth, and total schedule length.
    \item \textbf{Mapping overhead to effective noise/depth and simulatability.} We map compilation statistics into effective exposure measures and compare $(p_{\text{eff}}, D_H)$ against known noisy-IQP simulatability conditions.
\end{enumerate}

At this point, the analysis diverges into two complementary exposure metrics:

\begin{itemize}
    \item a \emph{global depth–noise score} \leo{this might be only narrative of conference submission} $\chi_H := p_{\rm eff}(H)\,D_H$ that summarizes architecture-dependent degradation in the $(D,p)$ phase diagram; and
    \item a \emph{support-resolved correlator-decay score} $\zeta_H := \max_j p_{S_j} d_{S_j}$ that captures worst-support damping hidden by global depth alone.
\end{itemize}

Together, these quantify how compilation reshapes the effective interaction hypergraph, including cases in which routing concentrates noise on specific high-weight supports even when $D_H$ remains modest. We make no claim that $\zeta_H$ directly certifies simulability; instead it \textcolor{red}{identifies architecture-induced loss of high-weight Pauli correlations that are necessary for IQP hardness but whose decay is not captured by global depth alone}\textcolor{green}{clarifies the role of $\zeta_H$ and avoids overstated hardness claims)}.

We summarize the paper’s contributions as:
\begin{enumerate}
    \item \textbf{A connectivity-aware framing of noisy IQP hardness.} We identify qubit connectivity and routing as decisive variables in the noisy-to-easy transition for IQP implementations.
    \item \textbf{A quantitative ``simulatability shift’’ methodology.} We provide a pipeline linking hardware graph, compilation overhead, and effective exposure measures $(\chi_H,\zeta_H)$ to known noisy-IQP thresholds.
    \item \textbf{Architecture-comparative predictions for IQP benchmarks.} Sparse-connectivity hardware induces both global depth inflation and worst-support correlator decay, while fully connected architectures mitigate both effects.
\end{enumerate}

IQP circuits have long been studied as restricted models capable of quantum advantage, while recent results clarify noise-induced efficient simulability. Our work lies at this intersection and highlights a systems-level factor that is typically implicit: the architecture-dependent compilation map from logical circuit to physical implementation. While compilation overhead is widely recognized as a practical concern, we argue it can be computationally decisive for assessing whether a noisy IQP experiment operates in the hard or the simulatable regime.

==> forJournal/previous_names.tex <==
\section{Results}
\label{sec:results}
We now evaluate the connectivity-induced simulatability shift $S(H)$ empirically across seven quantum computing platforms with publicly available information, validating the theoretical framework of Sec.~\ref{sec:methods} and quantifying the simulatability margin $m(H)$ for simulated noisy hardware devices. All experiments use $k{=}2$ (pairwise) interactions in a single IQP layer, since this setting already includes nontrivial IQP families relevant to near-term quantum advantage and captures the interaction structures studied in this work.

\subsection{Experimental Evaluation of Simulatability Margins}
\label{sec:phase-diagrams}

%%%% figure — hardware topologies (UNCHANGED)
\begin{figure}[t]
    \centering

    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/quantinuum_helios.pdf}
        \caption{Quantinuum Helios (98 qubits, all-to-all).}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/ionq_forte.pdf}
        \caption{IonQ Forte (36 qubits, all-to-all).}
    \end{subfigure}

    \vspace{1mm}

    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/google_willow.pdf}
        \caption{Google Willow (105 qubits, tapered triangular lattice).}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/google_sycamore.pdf}
        \caption{Google Sycamore (53 qubits, staggered nearest-neighbor lattice).}
    \end{subfigure}

    \vspace{1mm}

    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=0.88\linewidth]{paper_images/topologies/devices/rigetti_ankaa.pdf}
        \caption{Rigetti Ankaa-3 (82 qubits, defected rectangular grid).}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/ibm_washington.pdf}
        \caption{IBM Washington (127 qubits, heavy-hex connectivity).}
    \end{subfigure}

    \vspace{1mm}

    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/oqc_toshiko.pdf}
        \caption{OQC Toshiko (32 qubits, approx.\ sparse near-planar lattice).}
    \end{subfigure}

    \caption{Native hardware connectivity graphs used in the routing benchmark. The devices are ordered from fully connected trapped-ion architectures to more locality-constrained superconducting and planar-style layouts, illustrating the wide range of coupling structures that drive different routing overheads.}
    \label{fig:hardware_topologies}
\end{figure}

%%%%
\subsubsection{Compilation Setup}
We compile $k{=}2$ IQP circuits with a single IQP layer across four interaction patterns:
\begin{itemize}
    \item \textbf{Dense}: all pairwise interactions on $n{=}16$ qubits, giving $\binom{16}{2}=120$ terms.
    \item \textbf{Sparse}: a random subset of the $n{=}16$ pairwise interactions at density~$0.4$.
    \item \textbf{Local}: nearest-neighbor interactions on an $n{=}16$ qubit 1D chain, giving 15 terms.
    \item \textbf{RHG lattice}: interactions defined by a Raussendorf--Harrington--Goyal lattice~\cite{Raussendorf_2007}, the three-dimensional cluster-state topology used in topological measurement-based quantum computation.
\end{itemize}

For the dense, sparse, and local patterns, we use $n{=}16$ qubits in the phase-diagram study. For the RHG pattern, we additionally consider larger device-scale instances, since this interaction structure is of independent interest and remains hard to simulate under standard complexity-theoretic assumptions while requiring only $O(n)$ two-qubit gates~\cite{Fujii2016NoisyCommuting}. Specifically, we compile RHG circuits at $n{=}90$ ($2{\times}2{\times}2$ cells, 144 edges) and $n{=}127$ ($2{\times}2{\times}3$ cells, 208 edges).

From qiskit\cite{Qiskit} raw logical IQP circuit, compilation is performed in \texttt{pytket}~\cite{Sivarajah_2020}. For each hardware target $H$, we compute a hardware-constrained depth $D_H$ by routing on the coupling graph of $H$, rebasing to the target-family native gateset, and removing redundancies, together with a native fully connected baseline depth $D_{\mathrm{FC}}$ obtained by compiling the same logical circuit to the same native gateset without connectivity constraints. Here, depth denotes the abstract layer depth of the final compiled native circuit after routing and rebasing. This isolates topology-induced routing overhead from native-gateset effects and yields $\Delta D(H)=D_H-D_{\mathrm{FC}}$ as in Eq.~\eqref{eq:delta_depth}.
The native gate families used in the current experiments are: Quantinuum Helios $\{R_z,\mathrm{PhasedX},\mathrm{ZZPhase}\}$, IonQ Forte $\{\mathrm{GPI},\mathrm{GPI2},\mathrm{ZZPhase}\}$, Google devices $\{R_z,\mathrm{PhasedX}\text{-type},\mathrm{CZ},\mathrm{SYC}\}$ as available in the \texttt{pytket} version used for these experiments, Rigetti Ankaa-3 $\{R_z,\mathrm{RX},\mathrm{ISWAP}\}$, OQC Toshiko $\{R_z,\mathrm{SX},\mathrm{ECR}\}$, and IBM Washington $\{R_z,\mathrm{SX},X,\mathrm{CX}\}$.

\begin{comment} The gate sets are chosen to match the hardware families considered here: Quantinuum Helios uses $\{R_z,\mathrm{PhasedX},\mathrm{ZZPhase}\}$, IonQ Forte uses $\{\mathrm{GPI},\mathrm{GPI2},\mathrm{ZZPhase}\}$, Google devices use $\{R_z,\mathrm{PhasedXPow},\mathrm{SYC}/\mathrm{CZ}\}$, Rigetti Ankaa-3 uses $\{R_z,\mathrm{RX},\mathrm{ISWAP}\}$, and OQC Toshiko uses $\{R_z,\mathrm{SX},\mathrm{ECR}\}$. For IBM Washington, we use the Washington heavy-hex connectivity together with the IBM-native transpilation stack $\{R_z,SX,X,CX\}$.
%For realistic hardware targets, placement is performed on the full device graph rather than on a size-matched $n$-qubit subgraph.
\end{comment}

The hardware connectivity graphs used in these simulations are shown in Fig.~\ref{fig:hardware_topologies}. For Quantinuum Helios, IonQ Forte, Google Willow, Google Sycamore, IBM Washington, and Rigetti Ankaa-3, we use device layouts reconstructed from public vendor documentation, SDK coupling maps, or publicly released hardware diagrams. OQC Toshiko is the only exception: because we did not identify a public qubit-level coupling map for that processor, we model it with a sparse near-planar 32-qubit proxy architecture intended to capture the qualitative connectivity constraints of an OQC-style superconducting device. All results in this section are obtained in classical simulation of these connectivity and native-gate models.

Our work assumed an approximation of the effective noise parameter $p_{\mathrm{eff}}(H)$ with two-qubit gate error rates assigned from published or publicly available calibration proxies: Quantinuum Helios, $7.9 \times 10^{-4}$~\cite{ransford2025helios98qubittrappedionquantum}; IonQ Forte, $4.0 \times 10^{-3}$~\cite{ionqForteErrorRates}; Google Willow, $3.3 \times 10^{-3}$~\cite{googleWillowSpecSheet,google2024willow,google2025surfacecode}; Google Sycamore, $6.0 \times 10^{-3}$~\cite{arute2019quantum}; Rigetti Ankaa-3, $1.94 \times 10^{-2}$~\cite{rigetti_ankaa3}; OQC Toshiko, $4.6 \times 10^{-2}$~\cite{ward2026echocrossresonancegate}; and IBM Washington, $1.146 \times 10^{-2}$, taken from the median two-qubit error reported by "FakeWashingtonV2" and used here as a reproducible calibration proxy~\cite{qiskit_fake_washington}.



\subsubsection{Phase Diagram Results}

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/mean/phase_diagram_dense_k2_n16_layers1_samples5_mean.pdf}
        \caption{Dense (all $\binom{16}{2}=120$ interactions)}
        \label{fig:phase_dense}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/mean/phase_diagram_sparse_k2_n16_layers1_samples5_mean.pdf}
        \caption{Sparse (random subset, density~$0.4$)}
        \label{fig:phase_sparse}
    \end{subfigure}
    
    \vspace{0.27cm}
    
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/mean/phase_diagram_local_k2_n16_layers1_samples5_mean.pdf}
        \caption{Local (nearest-neighbor, 15 interactions)}
        \label{fig:phase_local}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/mean/phase_diagram_rhg_k2_n90_layers1_samples5_mean.pdf}
        \caption{RHG lattice ($n{=}90$, 144 interactions)}
        \label{fig:phase_rhg}
    \end{subfigure}
    
    \caption{Phase diagrams for $k{=}2$ IQP circuits across four interaction patterns. The critical boundary $D_*(p,k) = c/(p\ln(k/p))$ (black curve) separates the simulatable regime (teal, $m(H)<0$) from the potentially hard regime (coral, $m(H)>0$). Each platform is plotted at its operating point $(p_{\mathrm{eff}}(H), D_H)$; the legend reports the ideal fully-connected depth $D_{\mathrm{FC}}$ and the compiled depth $D_H$ as ($D_{\mathrm{FC}}$/$D_H$). Reported depths are sample means over five random circuit instances per interaction pattern, we also include standard deviations. The dense pattern~(a) represents a worst-case routing workload; the RHG lattice~(d) is a hardness-preserving interaction structure at device-relevant scale. Panels (a)--(c) use $n{=}16$ qubits; panel~(d) uses $n{=}90$.}
    \label{fig:phase_diagrams}
\end{figure*}


\begin{table}[h]
\centering
\footnotesize
\caption{Compiled depth $D_H$ for $k{=}2$, 1-layer IQP circuits across four interaction patterns. Dense, Sparse, and Local use $n{=}16$; RHG uses $n{=}90$ (only hardware with $\ge 90$ qubits shown). Entries are means over five random instances per pattern (depths rounded to nearest integer). Values in parentheses are the depth overhead $D_H/D_{\mathrm{ideal}}$ computed from the means.}
\label{tab:phase_summary}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l@{\hskip 6pt}r@{\hskip 6pt}r@{\hskip 6pt}r@{\hskip 6pt}r}
\toprule
\textbf{Platform} & \textbf{Dense} & \textbf{Sparse} & \textbf{Local} & \textbf{RHG} \\
\midrule
QTNM\ Helios  & 34\,(1.0$\times$) & 24\,(1.0$\times$) & 20\,(1.0$\times$) & 19\,(1.0$\times$) \\
IonQ Forte    & 47\,(1.0$\times$) & 36\,(1.0$\times$) & 33\,(1.0$\times$) & --- \\
Willow        & 674\,(2.8$\times$) & 383\,(2.3$\times$) & 126\,(1.0$\times$) & 614\,(5.3$\times$) \\
Sycamore      & 887\,(3.7$\times$) & 445\,(2.7$\times$) & 126\,(1.0$\times$) & --- \\
IBM Wash.     & 199\,(2.1$\times$) & 185\,(2.9$\times$) & 51\,(1.0$\times$) & 550\,(11.5$\times$) \\
Rigetti       & 279\,(3.1$\times$) & 138\,(2.3$\times$) & 48\,(1.0$\times$) & --- \\
OQC Toshiko   & 801\,(3.8$\times$) & 471\,(3.3$\times$) & 126\,(1.0$\times$) & --- \\

\bottomrule
\end{tabular}
\end{table}

Fig.~\ref{fig:phase_diagrams} visualizes the operating points $(p_{\mathrm{eff}}(H), D_H)$ relative to the critical boundary $D_*(p,k)$ from Eq.~\eqref{eq:critical_depth} for all four interaction patterns, and Table~\ref{tab:phase_summary} summarizes the compiled depths.

\paragraph{Dense interactions (worst case)}
The dense pattern includes all $\binom{16}{2}=120$ pairwise terms and produces the largest compilation cost. The two fully connected trapped-ion platforms already differ substantially in absolute compiled depth: Quantinuum Helios compiles to $D_H=34$ and IonQ Forte to $D_H=47$, both with zero routing overhead and within the critical boundary. Among the locality-constrained platforms, IBM Washington is the shallowest at $D_H=199$ ($2.1\times$ overhead), while Google Willow, Google Sycamore, Rigetti Ankaa-3, and OQC Toshiko reach $D_H=674$, $887$, $279$, and $801$, corresponding to $2.8\times$, $3.7\times$, $3.1\times$, and $3.8\times$ depth inflation over their native fully connected baselines.

\paragraph{Sparse and local interactions}
The sparse pattern reduces compiled depths relative to the dense case across all constrained architectures: for example, Google Willow drops from $674$ to $383$, Google Sycamore from $887$ to $445$, OQC Toshiko from $801$ to $471$, Rigetti Ankaa-3 from $279$ to $138$, and IBM Washington from $199$ to $185$. Quantinuum Helios and IonQ Forte remain routing-free and within the critical boundary at $D_H\approx24$ and $D_H\approx36$, respectively. For the local pattern, all platforms satisfy $D_H=D_{\mathrm{FC}}$, so no routing overhead is incurred. Because of low noise and native gatesets, the trapped-ion platforms are the only ones that remain inside the critical boundary.

\paragraph{RHG lattice (hardness-preserving, device-scale)}
The RHG lattice provides the strongest theoretical setting: $k{=}2$ interactions on this 3D topology are provably hard to simulate classically~\cite{Fujii2016NoisyCommuting}.
At $n{=}90$ (Fig.~\ref{fig:phase_diagrams}d), Quantinuum Helios achieves the shallowest depth, $D_H=19$, again with zero routing overhead. Google Willow and IBM Washington compile to $D_H=614$ and $D_H=550$, corresponding to $5.3\times$ and $11.5\times$ overhead over their native fully connected baselines, respectively. Other approximated hardwares are excluded here because of the $n{=}90$ qubit size required.
At $n{=}127$, only IBM Washington can accommodate the RHG instance among the hardware platforms considered, compiling to $D_H=1128$ with a $20.9\times$ depth overhead over its native fully connected baseline ($D_{\mathrm{ideal}}=54$). Both the $n=90$ and $n=127$ IBM RHG operating points lie well beyond the critical depth at the assumed error rate, illustrating that for current sparse-connectivity superconducting hardware the RHG interaction structure remains strongly routing-limited even though it uses only $O(n)$ two-qubit interactions.

\begin{comment}
\subsubsection{Phase Diagram Results}

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/phase_diagram_dense_k2_n16_layers1.pdf}
        \caption{Dense (all $\binom{16}{2}=120$ interactions)}
        \label{fig:phase_dense}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/phase_diagram_sparse_k2_n16_layers1.pdf}
        \caption{Sparse (random subset, density~$0.4$)}
        \label{fig:phase_sparse}
    \end{subfigure}
    
    \vspace{0.27cm}
    
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/phase_diagram_local_k2_n16_layers1.pdf}
        \caption{Local (nearest-neighbor, 15 interactions)}
        \label{fig:phase_local}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper_images/phase_diagram/phase_diagram_rhg_k2_n90_layers1.pdf}
        \caption{RHG lattice ($n{=}90$, 144 interactions)}
        \label{fig:phase_rhg}
    \end{subfigure}
    
    \caption{Phase diagrams for $k{=}2$ IQP circuits across four interaction patterns. The critical boundary $D_*(p,k) = c/(p\ln(k/p))$ (black curve) separates the simulatable regime (teal, $m(H)<0$) from the potentially hard regime (coral, $m(H)>0$). Each platform is plotted at its operating point $(p_{\mathrm{eff}}(H), D_H)$; the legend reports the ideal fully-connected depth $D_{\mathrm{FC}}$ and the compiled depth $D_H$ as ($D_{\mathrm{FC}}$/$D_H$). The dense pattern~(a) represents a worst-case routing workload; the RHG lattice~(d) is a hardness-preserving interaction structure at device-relevant scale. Panels (a)--(c) use $n{=}16$ qubits; panel~(d) uses $n{=}90$.}
    \label{fig:phase_diagrams}
\end{figure*}


\begin{table}[h]
\centering
\footnotesize
\caption{Compiled depth $D_H$ for $k{=}2$, 1-layer IQP circuits across four interaction patterns. Dense, Sparse, and Local use $n{=}16$; RHG uses $n{=}90$ (only hardware with $\ge 90$ qubits shown). Values in parentheses are the depth overhead $D_H/D_{\mathrm{ideal}}$.}
\label{tab:phase_summary}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l@{\hskip 6pt}r@{\hskip 6pt}r@{\hskip 6pt}r@{\hskip 6pt}r}
\toprule
\textbf{Platform} & \textbf{Dense} & \textbf{Sparse} & \textbf{Local} & \textbf{RHG} \\
\midrule
QTNM\ Helios  & 34\,(1.0$\times$) & 25\,(1.0$\times$) & 20\,(1.0$\times$) & 19\,(1.0$\times$) \\
IonQ Forte    & 47\,(1.0$\times$) & 38\,(1.0$\times$) & 33\,(1.0$\times$) & --- \\
Willow        & 674\,(2.8$\times$) & 448\,(2.6$\times$) & 126\,(1.0$\times$) & 614\,(5.3$\times$) \\
Sycamore      & 887\,(3.7$\times$) & 496\,(2.9$\times$) & 126\,(1.0$\times$) & --- \\
IBM Wash.     & 199\,(2.1$\times$) & 181\,(2.7$\times$) & 51\,(1.0$\times$) & 550\,(11.5$\times$) \\
Rigetti       & 279\,(3.1$\times$) & 128\,(2.0$\times$) & 48\,(1.0$\times$) & --- \\
OQC Toshiko   & 815\,(3.9$\times$) & 648\,(4.4$\times$) & 126\,(1.0$\times$) & --- \\

\bottomrule
\end{tabular}
\end{table}

Fig.~\ref{fig:phase_diagrams} visualizes the operating points $(p_{\mathrm{eff}}(H), D_H)$ relative to the critical boundary $D_*(p,k)$ from Eq.~\eqref{eq:critical_depth} for all four interaction patterns, and Table~\ref{tab:phase_summary} summarizes the compiled depths.

\paragraph{Dense interactions (worst case)}
The dense pattern includes all $\binom{16}{2}=120$ pairwise terms and produces the largest compilation cost. Under the current native-gateset model, the two fully connected trapped-ion platforms already differ substantially in absolute compiled depth: Quantinuum Helios compiles to $D_H=34$ and IonQ Forte to $D_H=47$, both with zero routing overhead and within the critical boundary. Among the locality-constrained platforms, IBM Washington is the shallowest at $D_H=199$ ($2.1\times$ overhead), while Google Willow, Google Sycamore, Rigetti Ankaa-3, and OQC Toshiko reach $D_H=674$, $887$, $279$, and $815$, corresponding to $2.8\times$, $3.7\times$, $3.1\times$, and $3.9\times$ depth inflation over their native fully connected baselines.


\paragraph{Sparse and local interactions}
The sparse pattern reduces compiled depths relative to the dense case across all constrained architectures: for example, Google Willow drops from $674$ to $448$, Google Sycamore from $887$ to $496$, OQC Toshiko from $815$ to $648$, Rigetti Ankaa-3 from $279$ to $128$, and IBM Washington from $199$ to $181$. Quantinuum Helios and IonQ Forte remain routing-free and within the critical boundary at $D_H=25$ and $D_H=38$, respectively. For the local pattern, all platforms satisfy $D_H=D_{\mathrm{FC}}$, so no routing overhead is incurred. Because of low noise and native gatesets, the trapped-ion platforms are the only ones that remain inside the critical boundary.

\paragraph{RHG lattice (hardness-preserving, device-scale)}
The RHG lattice provides the strongest theoretical setting: $k{=}2$ interactions on this 3D topology are provably hard to simulate classically~\cite{Fujii2016NoisyCommuting}, while requiring only $O(n)$ two-qubit gates.
At $n{=}90$ (Fig.~\ref{fig:phase_diagrams}d), Quantinuum Helios achieves the shallowest depth, $D_H=19$, again with zero routing overhead. Google Willow and IBM Washington compile to $D_H=614$ and $D_H=550$, corresponding to $5.3\times$ and $11.5\times$ overhead over their native fully connected baselines, respectively. Other approximated hardwares are excluded here because of the $n{=}90$ qubit size required.
At $n{=}127$, only IBM Washington can accommodate the RHG instance among the hardware platforms considered, compiling to $D_H=1128$ with a $20.9\times$ depth overhead over its native fully connected baseline ($D_{\mathrm{ideal}}=54$). Both the $n=90$ and $n=127$ IBM RHG operating points lie well beyond the critical depth at the assumed error rate, illustrating that for current sparse-connectivity superconducting hardware the RHG interaction structure remains strongly routing-limited even though it uses only $O(n)$ two-qubit interactions.


\end{comment}
\subsection{Compilation Overhead Scaling}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_dense.pdf}
        \caption{Dense: all $\binom{n}{2}$ interactions}
        \label{fig:ratio-dense}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_local.pdf}
        \caption{Local: nearest-neighbor only}
        \label{fig:ratio-local}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_sparse.pdf}
        \caption{Sparse: random $2n$ interactions}
        \label{fig:ratio-sparse}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_rhg.pdf}
        \caption{RHG lattice: $O(n)$ interactions ($n{=}18$--$127$)}
        \label{fig:ratio-rhg}
    \end{subfigure}
    
    \caption{Compilation efficiency $\eta_H := D_{\mathrm{FC}}/D_H$ versus qubit count for four interaction patterns. Solid segments correspond to compiled data; dashed segments show per-hardware linear extrapolations beyond the measured range. Panels~(a)--(c) use compiled data for $n=4$--$32$ and extrapolate to $n=70$; panel~(d) shows RHG lattice instances extrapoltions at the valid sizes $n\in\{18,44,90,127\}$.}

    \label{fig:compilation-overhead-scaling}
\end{figure}
\label{subsec:compilation_overhead}

\begin{figure}[t]
    \centering

    \begin{subfigure}[t]{0.31\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/line.pdf}
        \caption{Line: 1D nearest-neighbor chain.}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.31\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/ring.pdf}
        \caption{Ring: periodic 1D chain.}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.31\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/ladder.pdf}
        \caption{Ladder: quasi-1D two-rail lattice.}
    \end{subfigure}

    \caption{Reference connectivity graphs used as simplified baselines. These idealized low-dimensional topologies provide controlled comparisons against the native hardware layouts in Fig.~\ref{fig:hardware_topologies}.}
    \label{fig:reference_topologies}
\end{figure}

We empirically assess the connectivity-induced compilation overhead discussed in Sec.~\ref{sec:theory_DH_2D} by measuring the compilation efficiency as a function of qubit count.

\subsubsection{Setup}
For the dense, local, and sparse patterns, we compile IQP circuits for $n \in \{4,6,8,10,12,14,16,18,20,24,28,32\}$ across eleven connectivity graphs: the seven hardware targets of Fig.~\ref{fig:hardware_topologies}, plus fully connected, line, ring, and ladder reference topologies (Fig.~\ref{fig:reference_topologies}). For $n\le 12$ we generate five random instances per configuration; for $n\ge 14$ we generate three. For the RHG pattern, we compile the valid lattice sizes $n \in \{18,44,90,127\}$ with three random instances per size. The plotted efficiency ratio is depth-based,
\[
\eta_H := \frac{D_{\mathrm{FC}}}{D_H}.
\]

\subsubsection{Results}
Fig.~\ref{fig:compilation-overhead-scaling} shows $\eta_H$ versus $n$ for all four interaction patterns. For dense instances (Fig.~\ref{fig:ratio-dense}), the fully connected trapped-ion platforms remain at $\eta_H=1$ across the entire measured range, as expected from their all-to-all connectivity. By contrast, locality-constrained architectures show a clear degradation with increasing $n$. At $n=16$, the dense efficiencies already range from $\eta_H \approx 0.27$ for Google Sycamore to $\eta_H \approx 0.47$ for IBM Washington, with Google Willow, Rigetti Ankaa-3, and OQC Toshiko at approximately $0.35$, $0.32$, and $0.30$, respectively. By $n=32$, the separation is stronger still: Google Sycamore, Google Willow, IBM Washington, Rigetti Ankaa-3, and OQC Toshiko reach $\eta_H \approx 0.15$, $0.27$, $0.42$, $0.20$, and $0.14$, respectively.

For local patterns (Fig.~\ref{fig:ratio-local}), $\eta_H=1$ across all platforms and all measured qubit counts, consistent with the zero routing overhead observed in the phase-diagram analysis: nearest-neighbour interactions embed directly into every connectivity graph considered here. Sparse patterns (Fig.~\ref{fig:ratio-sparse}) interpolate between the dense and local extremes. At $n=16$, the constrained hardware efficiencies lie between roughly $0.31$ and $0.45$; by $n=32$ they fall further, to approximately $0.16$--$0.29$ across Google Willow, Google Sycamore, IBM Washington, Rigetti Ankaa-3, and OQC Toshiko.

The RHG pattern (Fig.~\ref{fig:ratio-rhg}) extends the analysis to device-relevant scales. At $n=18$, the fully connected platforms again remain at $\eta_H=1$, while the constrained hardware targets lie in the range $\eta_H \approx 0.44$--$0.55$. At $n=44$, Quantinuum Helios still remains at unity, while Google Willow, IBM Washington, Google Sycamore, and Rigetti Ankaa-3 drop to approximately $0.36$, $0.22$, $0.18$, and $0.30$, respectively. At $n=90$, only Quantinuum Helios ($\eta_H=1.0$), Google Willow ($\eta_H \approx 0.189$), and IBM Washington ($\eta_H \approx 0.087$) remain. At $n=127$, only IBM Washington can host the circuit among the constrained hardware platforms considered, with $\eta_H \approx 0.048$. The RHG trend is therefore especially informative at larger scales: although the interaction count remains only $O(n)$, embedding a three-dimensional interaction graph into low-dimensional hardware connectivity induces a strong routing penalty on sparse architectures.


\subsubsection{Implications for Simulatability}
These trends bear directly on the simulatability margin in Eq.~\eqref{eq:sim_margin}. As $\eta_H$ decreases, the compiled depth grows relative to the fully connected native baseline, tightening the effective noise budget compatible with $m(H)>0$. The phase-diagram analysis of Sec.~\ref{sec:phase-diagrams} shows that low routing overhead alone is not sufficient: Quantinuum Helios and IonQ Forte maintain $\eta_H=1$, above the critical boundary in the cases studied here, whereas several locality-constrained architectures remain in the simulatable regime even when the interaction pattern is relatively sparse. For RHG instances, sparse-connectivity hardware suffers increasingly severe depth inflation as the lattice size grows. Taken together, the overhead and phase-diagram results reinforce the same conclusion: near-term IQP advantage is favored by the combination of hardness-preserving low-$k$ interactions, low effective noise, and high connectivity.

\begin{comment}
\subsection{Compilation Overhead Scaling}

%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_dense.pdf}
        \caption{Dense: all $\binom{n}{2}$ interactions}
        \label{fig:ratio-dense}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_local.pdf}
        \caption{Local: nearest-neighbor only}
        \label{fig:ratio-local}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_sparse.pdf}
        \caption{Sparse: random $2n$ interactions}
        \label{fig:ratio-sparse}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{paper_images/compilation_overhead/ratio_vs_qubits_rhg.pdf}
        \caption{RHG lattice: $O(n)$ interactions ($n{=}18$--$127$)}
        \label{fig:ratio-rhg}
    \end{subfigure}
    
    \caption{Compilation efficiency $\eta_H := D_{\mathrm{FC}}/D_H$ versus qubit count for four interaction patterns. Solid segments correspond to compiled data; dashed segments show per-hardware linear extrapolations beyond the measured range. Panels~(a)--(c) use compiled data for $n=4$--$32$ and extrapolate to $n=70$; panel~(d) shows RHG lattice instances extrapoltions at the valid sizes $n\in\{18,44,90,127\}$.}

    \label{fig:compilation-overhead-scaling}
\end{figure}
\label{subsec:compilation_overhead}

\begin{figure}[t]
    \centering

    \begin{subfigure}[t]{0.31\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/line.pdf}
        \caption{Line: 1D nearest-neighbor chain.}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.31\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/ring.pdf}
        \caption{Ring: periodic 1D chain.}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.31\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{paper_images/topologies/devices/ladder.pdf}
        \caption{Ladder: quasi-1D two-rail lattice.}
    \end{subfigure}

    \caption{Reference connectivity graphs used as simplified baselines. These idealized low-dimensional topologies provide controlled comparisons against the native hardware layouts in Fig.~\ref{fig:hardware_topologies}.}
    \label{fig:reference_topologies}
\end{figure}

We empirically assess the connectivity-induced compilation overhead discussed in Sec.~\ref{sec:theory_DH_2D} by measuring the compilation efficiency as a function of qubit count.

\subsubsection{Setup}
For the dense, local, and sparse patterns, we compile IQP circuits for $n \in \{4,6,8,10,12,14,16,18,20,24,28,32\}$ across eleven connectivity graphs: the seven hardware targets of Fig.~\ref{fig:hardware_topologies}, plus fully connected, line, ring, and ladder reference topologies (Fig.~\ref{fig:reference_topologies}). For $n\le 12$ we generate five random instances per configuration; for $n\ge 14$ we generate three. For the RHG pattern, we compile the valid lattice sizes $n \in \{18,44,90,127\}$ with three random instances per size. The current native-compilation workflow is performed directly in \texttt{pytket}; the plotted efficiency ratio is depth-based,
\[
\eta_H := \frac{D_{\mathrm{FC}}}{D_H}.
\]


\subsubsection{Results}
Fig.~\ref{fig:compilation-overhead-scaling} shows $\eta_H$ versus $n$ for all four interaction patterns. For dense instances (Fig.~\ref{fig:ratio-dense}), the fully connected trapped-ion platforms remain at $\eta_H=1$ across the entire measured range, as expected from their all-to-all connectivity. By contrast, locality-constrained architectures show a clear degradation with increasing $n$. At $n=16$, the dense efficiencies already range from $\eta_H \approx 0.32$ for Google Sycamore to $\eta_H \approx 0.67$ for IBM Washington, with Google Willow, Rigetti Ankaa-3, and OQC Toshiko at approximately $0.40$, $0.37$, and $0.36$, respectively. By $n=32$, the separation is stronger still: Google Sycamore, Google Willow, IBM Washington, Rigetti Ankaa-3, and OQC Toshiko reach $\eta_H \approx 0.18$, $0.31$, $0.29$, $0.25$, and $0.19$, respectively.

For local patterns (Fig.~\ref{fig:ratio-local}), $\eta_H=1$ across all platforms and all measured qubit counts, consistent with the zero routing overhead observed in the phase-diagram analysis: nearest-neighbour interactions embed directly into every connectivity graph considered here. Sparse patterns (Fig.~\ref{fig:ratio-sparse}) interpolate between the dense and local extremes. At $n=16$, the constrained hardware efficiencies lie between roughly $0.40$ and $0.53$; by $n=32$ they fall further, to approximately $0.24$--$0.36$ across Google Willow, Google Sycamore, IBM Washington, Rigetti Ankaa-3, and OQC Toshiko.


The RHG pattern (Fig.~\ref{fig:ratio-rhg}) extends the analysis to device-relevant scales. At $n=18$, the fully connected platforms again remain at $\eta_H=1$, while the constrained hardware targets lie in the range $\eta_H \approx 0.55$--$0.66$. At $n=44$, Quantinuum Helios still remains at unity, while Google Willow, IBM Washington, Google Sycamore, and Rigetti Ankaa-3 drop to approximately $0.45$, $0.40$, $0.23$, and $0.24$, respectively. At $n=90$, only Quantinuum Helios ($\eta_H=1.0$), Google Willow ($\eta_H \approx 0.248$), and IBM Washington ($\eta_H \approx 0.172$) remain. At $n=127$, only IBM Washington can host the circuit among the constrained hardware platforms considered, with $\eta_H \approx 0.098$. The RHG trend is therefore especially informative at larger scales: although the interaction count remains only $O(n)$, embedding a three-dimensional interaction graph into low-dimensional hardware connectivity induces a strong routing penalty on sparse architectures.


\subsubsection{Implications for Simulatability}
These trends bear directly on the simulatability margin in Eq.~\eqref{eq:sim_margin}. As $\eta_H$ decreases, the compiled depth grows relative to the fully connected native baseline, tightening the effective noise budget compatible with $m(H)>0$. The phase-diagram analysis of Sec.~\ref{sec:phase-diagrams} shows that low routing overhead alone is not sufficient: Quantinuum Helios maintains $\eta_H=1$ and remains above the critical boundary in the cases studied here, whereas several locality-constrained architectures remain in the simulatable regime even when the interaction pattern is relatively sparse. For RHG instances, sparse-connectivity hardware suffers increasingly severe depth inflation as the lattice size grows. Taken together, the overhead and phase-diagram results reinforce the same conclusion: near-term IQP advantage is favored by the combination of hardness-preserving low-$k$ interactions, low effective noise, and high connectivity.
\end{comment}

\section{Discussion}
\label{sec:discussion}

Our empirical results support the framework of Sec.~\ref{sec:ciss}: limited connectivity increases compiled depth from the native fully connected baseline $D_{\mathrm{FC}}$ to the hardware-constrained depth $D_H$, thereby shifting noisy IQP implementations toward the efficiently simulatable regime. The key point is not only that current error rates are restrictive, but that connectivity multiplies the depth budget consumed by a circuit. Since the critical boundary depends inversely on noise, any connectivity-induced inflation of $D_H$ translates directly into a stricter noise requirement for retaining a positive simulatability margin.


\subsection{Connectivity Penalty and Noise Budget}

A central outcome of the phase-diagram analysis is that connectivity matters by converting a given native fully connected depth $D_{\mathrm{FC}}$ into a larger hardware-constrained depth $D_H$. This depth inflation reduces the noise budget compatible with $m(H)>0$. For the local pattern, where routing overhead vanishes and $D_H=D_{\mathrm{FC}}$, all constrained superconducting platforms already lie in the simulatable regime: for example, Willow has $D_H=185$ while $D_*(p_{\mathrm{Willow}},2)\approx 47$, IBM Washington has $D_H=127$ while $D_*(p_{\mathrm{IBM}},2)\approx 17$, and OQC Toshiko has $D_H=202$ while $D_*(p_{\mathrm{OQC}},2)\approx 6$. Thus, current noise levels alone are already sufficient to place these platforms below the critical boundary even before routing overhead is introduced.

Connectivity then worsens this picture substantially for less structured interaction patterns. In the dense $n=16$ instance, the compiled depth rises from $D_{\mathrm{FC}}=353$ to $D_H=887$ for Willow, from $239$ to $359$ for IBM Washington, from $147$ to $396$ for Rigetti Ankaa-3, and from $356$ to $989$ for OQC Toshiko. These factors of $1.5\times$ to $2.8\times$ represent a direct connectivity penalty. Since the critical depth scales as $D_*(p,k)\sim 1/p$, such inflation implies that the tolerable effective noise rate must decrease by the same factor in order to preserve the same margin.

Among the platforms considered, Quantinuum Helios is the clearest positive-margin case, while IonQ Forte is near the boundary. These results indicate that connectivity alone is not sufficient, and sparse connectivity still tightens the noise threshold for retaining hardness.



\subsection{Gate Speed versus Computational Hardness}

Superconducting platforms can execute two-qubit gates much faster than trapped-ion platforms~\cite{chen2025efficient, schafer2018fast, bruzewicz2019trapped}, but gate speed is not the quantity relevant to the simulatability boundary considered here. The relevant distinction is whether the compiled noisy circuit lies in the regime $m(H)<0$, where efficient classical approximation is expected, or in the regime $m(H)>0$, where classical simulation is conjecturally hard.

Our results show that fast execution does not compensate for depth inflation combined with finite noise. In the presented experiments, the constrained superconducting platforms remain in the simulatable regime even when routing overhead is absent, and move further into that regime once connectivity-induced compilation overhead is introduced. By contrast, the approximated Quantinuum Helios maintains positive margin in the tested instances because it combines low effective noise with zero routing overhead. The relevant resource for retaining advantage is therefore not raw gate speed but the ability to keep the compiled depth below the critical boundary.


\subsection{Scaling to $\mathcal{O}(10^2)$ Qubits}

The depth-scaling data in Fig.~\ref{fig:compilation-overhead-scaling} show that the connectivity penalty becomes more severe as system size increases. For dense instances, the fully connected platforms remain at $\eta_H=D_{\mathrm{FC}}/D_H=1$, while constrained architectures fall steadily below unity; by $n=32$, the dense efficiencies are approximately $0.31$ for Willow, $0.29$ for IBM Washington, $0.25$ for Rigetti Ankaa-3, $0.19$ for OQC Toshiko, and $0.18$ for Sycamore. For RHG instances, the effect is even clearer at larger scales: at $n=90$, Willow and IBM Washington fall to $\eta_H\approx 0.248$ and $0.172$, and at $n=127$ IBM Washington reaches $\eta_H\approx 0.098$.

Because $\eta_H=D_{\mathrm{FC}}/D_H$, any reduction in $\eta_H$ means that the hardware-constrained circuit consumes a larger fraction of the available depth budget than its fully connected counterpart. Equivalently, maintaining the same simulatability margin requires a correspondingly smaller effective noise rate according to Eq.~(\ref{eq:noise_budget_ratio}). Connectivity therefore acts as a multiplicative penalty on the tolerable noise threshold.

For current sparse-connectivity platforms, this penalty becomes substantial at device-relevant scales. In the RHG setting, IBM Washington reaches $D_H=693$ at $n=90$ and $D_H=1372$ at $n=127$, far above its native fully connected baselines of $119$ and $135$. Thus, even when the logical interaction structure uses only $O(n)$ two-qubit terms, the hardware embedding cost can dominate the compiled depth. This suggests that sparse-connectivity platforms face a shrinking pre-fault-tolerant window for IQP-based advantage, reducing noise helps, but connectivity-induced depth inflation simultaneously tightens the level of noise reduction required.

% \subsection{Algorithm-Hardware Co-Design}

% The stark contrast between dense and local patterns (Figs.~\ref{fig:ratio-dense}, \ref{fig:ratio-local}) suggests a mitigation strategy: designing IQP instances whose interaction hypergraph $G_C$ (cf. Sec.~\ref{sec:ciss}) matches the hardware connectivity graph $H$. When $G_C \subseteq H$, routing is eliminated and $D_H = D_{\mathrm{ideal}}$.

% This approach has precedent in variational algorithms for local Hamiltonians and QAOA on bounded-degree graphs. For IQP circuits, restricting to $k$-local terms with geometrically local support on a 2D grid would achieve $\mathrm{diam}_{\mathrm{2D}}(s) = O(1)$ in Eq.~\eqref{eq:term_depth_lower}, eliminating the depth overhead.

% However, our results reveal a fundamental limitation of this strategy for current superconducting devices: even with zero routing overhead, the local pattern yields $m(H) < 0$ for all five superconducting platforms (e.g., $m \approx -30$ for Willow, $m \approx -99$ for IBM). The depth budget consumed by native gate synthesis alone already exceeds $D_*(p,k)$ at current noise levels. Thus, hardware-native interaction patterns are necessary but not sufficient; error-rate reduction remains essential.

% Moreover, such restrictions may affect hardness guarantees. The simulatability result of~\cite{rajakumar2025polynomial} applies to general $k$-local IQP circuits; whether topology-restricted subfamilies retain worst-case hardness is an open question requiring separate analysis.

\subsection{Noise Model Limitations}

Our analysis uses $p_{\mathrm{eff}}(H)$ as a simplified effective-noise proxy based primarily on reported two-qubit gate error rates. This is a useful first-order choice, but the total noise affecting a compiled IQP circuit is not limited to two-qubit errors alone.

Connectivity-constrained compilation can also amplify memory errors through longer circuit duration and idle time, and can worsen crosstalk; these effects compound the usual SPAM and one-qubit contributions already present in the device error budget~\cite{cowtan2019qubit, das2021adapt, rudinger2021experimental, bravyi2021mitigating}. Accordingly, the connectivity-induced shift in simulatability should be interpreted as arising from overall noise exposure, with the present $p_{\mathrm{eff}}(H)$ serving as an approximate proxy. An important direction for future work is to extend this framework to broader error models and real quantum devices, and to integrate error mitigation and pre-fault-tolerant error-suppression techniques in order to study how they modify the estimation of $p_{\mathrm{eff}}(H)$ and the resulting simulatability margins~\cite{Cai_2023, placidi2026deeplearningapproachesquantum, Cirstoiu_2023}. While such methods may improve the effective operating point, they do not eliminate the routing-induced depth overhead associated with limited connectivity.




\section{Conclusion}
\label{sec:conclusion}

We have systematically analyzed the connectivity-induced simulatability shift for noisy IQP circuits, connecting the theoretical framework of~\cite{rajakumar2025polynomial} to empirical compilation data across seven quantum platforms.

% Our main contributions are:
% \begin{enumerate}
%     \item \textbf{Empirical validation of depth overhead bounds}: Compilation experiments at $n{=}16$ confirm that superconducting platforms incur $D_H/D_{\mathrm{ideal}} = 2.7$--$5.1\times$ depth overhead for dense interactions, scaling toward the $O(\sqrt{n})$ bound of Eq.~\eqref{eq:DH_2D_upper}. For hardness-preserving RHG lattice interactions at device-relevant scales ($n{=}90$--$127$), overhead ratios reach $7.7$--$10.5\times$.
    
%     \item \textbf{Quantification of simulatability margins}: Using the phase-diagram framework of Sec.~\ref{sec:ciss}, we showed that trapped-ion platforms maintain positive margin $m(H) > 0$ at current noise levels across all interaction patterns, while \emph{all} superconducting platforms yield $m(H) < 0$ for every pattern, including local interactions with zero routing overhead. The dominant factor is the effective noise strength: superconducting critical depths $D_*(p,k)$ range from $\approx 6$ (OQC) to $\approx 47$ (Willow), which even the shallowest routing-free circuits exceed.
    
%     \item \textbf{Noise budget ratio analysis}: Per Eq.~\eqref{eq:noise_budget_ratio}, the noise tolerance for maintaining hardness scales inversely with depth overhead. Superconducting platforms would require $p_{\mathrm{eff}} \lesssim 2 \times 10^{-3}$ to achieve $m(H) > 0$ even with ideal connectivity, and $p_{\mathrm{eff}} \lesssim 10^{-4}$ after routing, approaching fault-tolerant thresholds.
% \end{enumerate}
Our compilation experiments show that connectivity induces a concrete depth penalty that becomes more severe as the system scales. For dense $k=2$ IQP circuits, fully connected platforms retain $D_{\mathrm{FC}}/D_H = 1$, whereas locality-constrained architectures exhibit progressively smaller efficiency as $n$ grows. By $n=32$, the dense depth efficiencies are approximately $0.31$ for Willow, $0.29$ for IBM Washington, $0.25$ for Rigetti Ankaa-3, $0.19$ for OQC Toshiko, and $0.18$ for Sycamore. For RHG lattice instances, the same effect persists at device-relevant scales: at $n=90$, Willow and IBM Washington drop to $D_{\mathrm{FC}}/D_H \approx 0.248$ and $0.172$, and at $n=127$ IBM Washington reaches $0.098$.

The phase-diagram analysis indicates that, under the present effective-noise model, the constrained superconducting platforms already lie in the simulatable regime for the tested patterns, including the local case where routing overhead vanishes. The role of connectivity is therefore not to create this limitation on its own, but to exacerbate it by inflating $D_H$ relative to $D_{\mathrm{FC}}$, which in turn tightens the effective noise threshold required to retain a positive simulatability margin. In this sense, connectivity acts as a multiplicative penalty on the noise budget for advantage retention. Fully connected platforms avoid this routing-induced depth inflation, although positive margin still depends on the combination of connectivity, native compilation cost, and effective noise rate.

These results support the central claim of this work: connectivity is a direct limit on actionable quantum advantage in noisy IQP circuits. Sparse connectivity increases compiled depth, and because the critical boundary scales inversely with noise, this depth inflation forces a correspondingly lower hardware noise rate to preserve hardness. In this sense, connectivity and noise must be treated jointly, reducing noise helps, but poor connectivity simultaneously increases the level of noise suppression required.

More broadly, the phase-diagram methodology developed here provides a practical way to connect hardware compilation data to noise-dependent simulatability criteria. Although this work focuses on IQP circuits, the same methodology can be applied to other circuit families whenever a noise-dependent classical simulatability boundary is available.



==> forJournal/someleonotes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\leo{for appendix or notes}
\section{Experimental validation and computability}
\label{sec:experiments_and_computability}
\leo{this is undergoing analysis, I am designing the experiments and see what I can compute}
\paragraph{Quantities that are always computable}

For any hardware $H$ and compiler,
the following quantities are directly computable
from the scheduled compiled circuit $\widetilde{C}_H$
and require \emph{no noise model}:
\begin{itemize}
    \item global two-qubit depth $D_H$,
    \item global exposure depth $d_{\mathrm{eff}}(H)=D_H$,
    \item per-support depths $d_{S_j}$ from
    Eq.~\eqref{eq:dsj} (with $\eta=0$ if idle
    is not included),
    \item worst-support depth $d_{\max}(H)$,
    \item architecture-only ratios
    $D_{FC}/D_H$ and
    $d_{\max}^{FC}/d_{\max}(H)$.
\end{itemize}
These provide the purely geometric penalties
in Eqs.~\eqref{eq:noise_budget_ratio}
and~\eqref{eq:local_ratio},
independent of calibration data.

\paragraph{Device-dependent indicators.}

To evaluate $\chi_H$, $\zeta_H$,
and $\mathcal{I}_H$
in Eqs.~\eqref{eq:chiH}–\eqref{eq:hardness_indicator},
a noise model must be supplied:
\begin{itemize}
    \item two-qubit error-per-gate (EPC)
    and $T_2$ times for superconducting devices
    (e.g.\ IBM),
    \item two-qubit depolarizing estimates and
    coherence times for trapped-ion devices
    (e.g.\ Quantinuum),
    \item scheduled gate durations to compute
    idle exposure $t_q^{(\mathrm{idle})}$,
    \item optional cross-talk or leakage parameters
    if available.
\end{itemize}
These determine $p_{\mathrm{eff}}(H)$
and $p_{S_j}$ in Eq.~\eqref{eq:psj}.
\leo{changing this atm}


\paragraph{Experiments.}
All experimental components in this work fall into four stages.

\begin{enumerate}
\item \textbf{Instance generation.}
Construct families of $n$-qubit, $k$-local IQP circuits with controlled support structure:
(i) random nonlocal supports,
(ii) geometrically local supports,
(iii) mixed-support families with a tunable fraction of long-range $S_j$.
Record all supports and angles, and obtain the ideal depth $D_{\mathrm{ideal}}$ by compiling to an all-to-all coupling map in the same native basis.
\leo{Purpose: create circuit families where we explicitly control the presence or absence of long-range supports, enabling clean comparison of global and support-level effects.}

\item \textbf{Multi-architecture compilation.}
For each instance and connectivity graph $H\in\{H_{\mathrm{FC}},H_{\mathrm{IBM}},H_{\mathrm{2D}},H_{\mathrm{line}}\}$, compile to obtain $\widetilde{C}_H$.  
Extract the global depth $D_H$, depth inflation $\Delta D(H)$, all support-level exposures $\{d_{S_j}\}$, and the worst-support value $d_{\max}(H)$.
\leo{Purpose: explicitly quantify how topology modifies depth, routing, and exposure; these measurements feed all subsequent experiments involving $\chi_H$, $\zeta_H$, and their ratios.}

\item \textbf{Global and local exposure analysis (core plots).}
Using calibration data for each target backend, compute the global exposure $\chi_H=p_{\mathrm{eff}}(H)D_H$ and the support-resolved exposures $\Lambda_j=p_{S_j}d_{S_j}$, together with the worst-support value $\zeta_H=\max_j\Lambda_j$.  
Produce:
(a) global phase-diagram plots $(p_{\mathrm{eff}},D_H)$ marking the shift from $(D_{\mathrm{ideal}},p_{\mathrm{ideal}})$,  
(b) depth-inflation ratios $D_H/D_{\mathrm{ideal}}$,  
(c) worst-support exposure histograms, and  
(d) scatter plots comparing $\chi_H$ vs.\ $\zeta_H$ across architectures.
\leo{Purpose: these plots show how routing and topology move circuits within the known global depth–noise phase diagram, and how certain supports incur disproportionately large coherence loss.}

\item \textbf{Correlation-decay validation and simulability proxies.}
For selected supports $S_j$ (typically those with largest $d_{S_j}$ under sparse topologies), prepare states on hardware and measure $\langle X_{S_j}\rangle$ as a function of circuit truncation, noise scaling, or synthetic depolarization.  
Fit the empirical decay to $\exp(-\Lambda_j)$ and verify alignment with the predicted $p_{S_j}d_{S_j}$.  
Complement this with classical simulation benchmarks (exact simulation or tensor-network approximations) comparing runtime or sampling error across hardware-induced compilations.
\leo{Purpose: validate that $\Lambda_j$ captures real correlator decay, and connect this decay pattern to empirical changes in classical simulability.}
\end{enumerate}

\paragraph{Suggested visualizations.}
For clarity and reproducibility, the paper will include:  
(i) a 2D phase diagram showing per-architecture arrows from $(D_{\mathrm{ideal}},p_{\mathrm{ideal}})$ to $(D_H,p_{\mathrm{eff}}(H))$;  
(ii) bar/violin plots of $D_H/D_{\mathrm{ideal}}$ across topologies;  
(iii) worst-support exposure curves $d_{\max}(H)$ and $\zeta_H$ across $H$;  
(iv) correlation-decay fits demonstrating empirical agreement with Eq.~\eqref{eq:correlator_decay};  
(v) scatter plots comparing $\chi_H$ and $\zeta_H$ as a function of connectivity class.


\leo{An example to motivate why we need the two approaches}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Worked examples: when the global margin $m(H)$ suffices vs.\ when the
structure-aware margin $m_\zeta(H)$ is necessary}
\label{subsub:worked_examples_m_vs_mzeta}

We give two explicit IQP constructions illustrating the two degradation
mechanisms introduced above.  In both examples we work with an IQP family
\begin{equation}
C(\bm\theta)
\;=\;
\prod_{j=1}^{M}\exp\!\bigl(i\theta_j X_{S_j}\bigr),
\qquad
S_j\subseteq[n],\ \ |S_j|\le k,
\label{eq:iqp_family_general}
\end{equation}
where all $X_{S_j}$ commute.  We consider a compiled physical circuit
$\widetilde{C}_H$ on a hardware graph $H$ with scheduled two-qubit depth $D_H$.
Noise is treated at the level of the abstract parameter $p$ appearing in the
noisy-IQP critical-depth boundary $D_\ast(p,k)$ \cite{Bremner_2017}, and is
instantiated by a compilation-dependent effective noise $p_{\mathrm{eff}}(H)$.

\paragraph{Noise bookkeeping on a schedule: why $p_{S}$ and $d_S$ appear}
Fix a logical interaction support $S\subseteq[n]$.  During compilation, gates and
idles affecting qubits in $S$ occur over a finite window of the schedule (from
the first to the last moment any qubit in $S$ is involved in realizing that
logical interaction).  Let $L_S^{(2q)}$ be the number of scheduled two-qubit
layers within that window that touch at least one qubit in $S$, and let
$L_S^{(\mathrm{idle})}$ be the number of scheduled layers in which at least one
qubit in $S$ is idle while other qubits are active.  We set
\begin{equation}
d_{S}
:= D^{(2q)}_{S} + \eta\, D^{(\mathrm{idle})}_{S},
\label{eq:def_dS_example}
\end{equation}
so $d_S$ counts how long the support is ``exposed'' to entangling noise plus (a
weighted amount of) idle dephasing.

To connect exposure to correlator attenuation, assume a simple local model:
each two-qubit gate acting on qubits that intersect $S$ fails independently with
probability $\epsilon_{2q}$ (after compilation, including SWAP decompositions),
and idling of a qubit $q\in S$ for time $t$ induces dephasing
$\exp(-t/T_{2,q})$ in the $X$ basis.  If the schedule induces
$N_S^{(2q)}$ such two-qubit gates touching $S$ and total idle times
$\{t_q^{(\mathrm{idle})}\}_{q\in S}$ over the window, then the probability that
pm \emph{no} error affects $S$ during the window is approximated by
\begin{equation}
P(\text{no error on }S)
\;\approx\;
(1-\epsilon_{2q})^{N_S^{(2q)}}\,
\prod_{q\in S} e^{-t_q^{(\mathrm{idle})}/T_{2,q}}.
\label{eq:no_error_on_S}
\end{equation}
Accordingly, the accumulated error probability on $S$ is
\begin{equation}
p_S
\;:=\;
1 - P(\text{no error on }S)
\;\approx\;
1-(1-\epsilon_{2q})^{N_S^{(2q)}}\prod_{q\in S} e^{-t_q^{(\mathrm{idle})}/T_{2,q}}.
\label{eq:def_pS_example}
\end{equation}
For small errors, use $(1-\epsilon)^{N}\approx e^{-\epsilon N}$ to obtain the
first-order scaling
\begin{equation}
p_S
\;\approx\;
1-\exp\!\Bigl(-\epsilon_{2q}N_S^{(2q)}-\sum_{q\in S}t_q^{(\mathrm{idle})}/T_{2,q}\Bigr)
\;\approx\;
\epsilon_{2q}N_S^{(2q)}+\sum_{q\in S}t_q^{(\mathrm{idle})}/T_{2,q}.
\label{eq:pS_first_order}
\end{equation}
This is the (minimal) motivation for using support-specific quantities
$p_S$ and $d_S$: routing and scheduling can make $(N_S^{(2q)},t_q^{(\mathrm{idle})})$
\emph{highly non-uniform} over supports even when the global depth $D_H$ is modest.

Finally, under standard Pauli-noise heuristics, the $X$-correlator on $S$
attenuates approximately exponentially in the exposure:
\begin{equation}
\langle X_S\rangle_{\mathrm{noisy}}
\;\approx\;
\langle X_S\rangle_{\mathrm{ideal}}
\exp\!\bigl(-\Lambda_S\bigr),
\qquad
\Lambda_S := p_S\,d_S,
\label{eq:correlator_decay_example}
\end{equation}
and the worst-support decay score and margin are
\begin{equation}
\zeta_H := \max_j \Lambda_{S_j},
\qquad
m_\zeta(H) := \tau_\zeta-\zeta_H.
\label{eq:zeta_and_margin_example}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection*{Example A (global-depth dominated): uniform local supports}
\label{subsub:example_global}

Consider $n$ qubits arranged on the same connectivity as the hardware (e.g., a
2D grid), and an IQP instance consisting only of geometrically local two-body
terms scheduled as disjoint matchings:
\begin{equation}
C_{\mathrm{local}}
=
\prod_{t=1}^{L}
\left(
\prod_{(u,v)\in M_t}
\exp(i\theta_{uv}^{(t)} X_uX_v)
\right),
\label{eq:iqp_local_matching}
\end{equation}
where each $M_t$ is a matching of \emph{nearest-neighbor} edges in $H$, so all
two-qubit interactions in a layer are implementable in parallel without routing.

\paragraph{Compilation and exposure}
Because interactions are already local, compilation inserts essentially no SWAPs
and preserves the schedule up to constants:
\begin{equation}
D_H \approx D_{\mathrm{ideal}} = L.
\label{eq:DH_local}
\end{equation}
Moreover, every support is size $|S|=2$ and experiences comparable exposure:
for each $(u,v)\in M_t$,
\begin{equation}
d_{\{u,v\}} = \Theta(1),\qquad
N_{\{u,v\}}^{(2q)}=\Theta(1),\qquad
t_u^{(\mathrm{idle})},t_v^{(\mathrm{idle})}=\Theta(1),
\label{eq:uniform_support_exposure}
\end{equation}
so $p_{\{u,v\}}=\Theta(\epsilon_{2q})$ and hence
\begin{equation}
\Lambda_{\{u,v\}} = p_{\{u,v\}}d_{\{u,v\}}=\Theta(\epsilon_{2q}),
\qquad
\zeta_H=\Theta(\epsilon_{2q}).
\label{eq:zeta_small_local}
\end{equation}
Thus for realistic parameters one can have $m_\zeta(H)>0$ while the circuit
becomes globally simulatable simply by increasing the number of layers $L$.

\paragraph{Global-margin transition}
If $L$ is increased at fixed $p_{\mathrm{eff}}(H)$ until
\begin{equation}
m(H)=D_\ast\!\bigl(p_{\mathrm{eff}}(H),k\bigr)-D_H<0,
\label{eq:global_margin_negative_example}
\end{equation}
then the known noisy-IQP sufficient condition predicts entry into the efficient
classical simulation regime \cite{Bremner_2017}.  In this regime the degradation
is \emph{global}: there is no single ``bad'' support; rather, the overall depth
exceeds the critical scale.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection*{Example B (structure-dominated): one stretched nonlocal support}
\label{subsub:example_structure}

We now construct an IQP instance for which the \emph{global} schedule remains
shallow (so $m(H)$ can stay positive), yet a single interaction support becomes
overdamped by routing and idling (so $m_\zeta(H)$ turns negative).

\paragraph{Circuit family.}
Fix $k\ge 3$ constant.  Let $S=\{s_1,\dots,s_k\}$ be a $k$-tuple of qubits placed
far apart on a 2D grid embedding, with diameter
\begin{equation}
\mathrm{diam}_{\mathrm{2D}}(S)
:= \max_{a,b\in S}\mathrm{dist}_{\mathrm{2D}}(a,b)
= \Theta(\sqrt{n}).
\label{eq:diam_large}
\end{equation}
Consider the IQP instance with just \emph{two} commuting generators:
\begin{equation}
C_{\mathrm{stretched}}
:= \exp(i\theta X_{S})\,\exp(i\phi X_{T}),
\label{eq:iqp_stretched}
\end{equation}
where $T\subseteq[n],\ |T|\le k,\ \mathrm{diam}_{\mathrm{2D}}(T)=O(1)$. $T$ is a local support (added only so the circuit is not ``one-term'' and
to emphasize that only $S$ is problematic).  The logical depth
$D_{\mathrm{ideal}}$ under full connectivity is $O(1)$, and the compiled depth
$D_H$ remains $O(1)$ in the sense of ``number of logical layers'' even though
routing is required inside the synthesis of the $k$-body term.

\paragraph{Sketch of a standard synthesis and why one support gets long exposure}
A typical synthesis of $\exp(i\theta X_S)$ uses a parity-compute / phase /
uncompute pattern: compute the parity of $X$ on all qubits in $S$ onto a chosen
pivot qubit $s_1$ via a CNOT tree, apply a one-qubit $R_Z(2\theta)$ on the pivot
in the appropriate basis, then uncompute.  On a fully connected device, the CNOT
tree can be scheduled in $O(\log k)$ depth (or $O(k)$ with a line), which is
still $O(1)$ for constant $k$.  On a 2D grid with \emph{geometrically stretched}
$S$, however, each interaction needed for parity accumulation requires bringing
qubits together through SWAP routing across distances $\Theta(\sqrt{n})$.

Concretely, any procedure that propagates parity information across the support
must communicate across the diameter \eqref{eq:diam_large}.  Therefore there is
a constant $c>0$ (independent of $n$) such that the two-qubit depth contributed
by implementing the single term on $S$ obeys the lower bound
\begin{equation}
d_S \;\ge\; c\,\mathrm{diam}_{\mathrm{2D}}(S) \;=\; \Theta(\sqrt{n}),
\label{eq:dS_lower_sqrt_n}
\end{equation}
which is exactly the support-diameter mechanism discussed in
Sec.~\ref{sec:theory_DH_2D}.  In addition, because routing occupies intermediate
qubits while waiting for remote qubits to arrive, the window typically induces
idle exposure on some qubits in $S$, so $L_S^{(\mathrm{idle})}$ and
$\sum_{q\in S}t_q^{(\mathrm{idle})}/T_{2,q}$ can scale similarly with
$\sqrt{n}$.

\paragraph{From routing to correlator suppression on the stretched support.}
Assume for simplicity homogeneous parameters
$T_{2,q}=T_2$ and per-two-qubit-gate error $\epsilon_{2q}$.  The number of
two-qubit gates touching $S$ during the window is at least linear in the
routing depth, hence
\begin{equation}
N_S^{(2q)} \;=\; \Omega(d_S) \;=\; \Omega(\sqrt{n}).
\label{eq:NS_lower}
\end{equation}
Using the first-order approximation \eqref{eq:pS_first_order} and absorbing idle
terms into the same scaling (worst case), we obtain
\begin{equation}
p_S \;\gtrsim\; c_1\,\epsilon_{2q}\sqrt{n} \;+\; c_2\,\frac{\sqrt{n}\,t_{\mathrm{layer}}}{T_2}
\;=\; \Theta(\sqrt{n})\cdot
\left(\epsilon_{2q}+\frac{t_{\mathrm{layer}}}{T_2}\right),
\label{eq:pS_sqrt_n}
\end{equation}
where $t_{\mathrm{layer}}$ is a characteristic layer time.  Combining with
$d_S=\Theta(\sqrt{n})$ yields the stretched-support decay exponent
\begin{equation}
\Lambda_S = p_S\,d_S
\;\gtrsim\;
\Theta(n)\cdot
\left(\epsilon_{2q}+\frac{t_{\mathrm{layer}}}{T_2}\right).
\label{eq:Lambda_scaling_n}
\end{equation}
Consequently,
\begin{equation}
\langle X_S\rangle_{\mathrm{noisy}}
\approx
\langle X_S\rangle_{\mathrm{ideal}}e^{-\Lambda_S}
\;\le\;
\langle X_S\rangle_{\mathrm{ideal}}
\exp\!\left[-\Theta(n)\!\left(\epsilon_{2q}+\frac{t_{\mathrm{layer}}}{T_2}\right)\right],
\label{eq:XS_exponentially_small}
\end{equation}
which becomes exponentially small in $n$ even if the \emph{global} compiled depth
$D_H$ (as ``number of logical layers'') is still $O(1)$.

\paragraph{Why this can imply effective simulability even when $m(H)>0$}
In this construction the output distribution is controlled by Fourier
coefficients of the form $\langle X_{S'}\rangle$ for various supports $S'$
(precisely which coefficients matter depends on the observable / estimator being
used).  When the worst stretched support $S$ is overdamped, its high-weight
correlation effectively vanishes and the implemented circuit behaves like a
\emph{different} IQP instance in which the corresponding generator is removed or
replaced by a much smaller effective angle.  Operationally, the hardware is no
longer sampling from the intended hard instance but from a ``pruned'' one with
suppressed high-weight Pauli structure, which is exactly the type of structural
degradation that simulatability mechanisms exploit (suppression of high-weight
Pauli correlations and loss of anticoncentration) \cite{Bremner_2017, Napp_2022, Bravyi2022}.

A simple experimental sketch that exposes this failure mode is:
\begin{enumerate}
\item Choose $S=\{s_1,\dots,s_k\}$ with large grid diameter and a control support
$T$ with small diameter.
\item Implement $C_{\mathrm{stretched}}$ on hardware and measure $\langle X_S\rangle$
and $\langle X_T\rangle$ directly by appending $H^{\otimes n}$ at the end and
estimating the corresponding parity in the $Z$ basis.
\item Observe that $\langle X_T\rangle$ remains appreciable while
$\langle X_S\rangle$ decays rapidly with $n$ (or with increased routing), in
accordance with \eqref{eq:XS_exponentially_small}.
\end{enumerate}
This demonstrates that a single support can lose the multi-qubit coherence
needed to realize the intended IQP correlations even though the global operating
point $(D_H,p_{\mathrm{eff}})$ remains below the coarse boundary $D_\ast(p,k)$.

\paragraph{Margins in this example}
Because the overall instance uses only $O(1)$ logical layers, one may have
\begin{equation}
m(H)=D_\ast\!\bigl(p_{\mathrm{eff}}(H),k\bigr)-D_H>0,
\label{eq:m_positive_structure_example}
\end{equation}
while the worst-support exponent \eqref{eq:Lambda_scaling_n} exceeds the
correlator threshold:
\begin{equation}
m_\zeta(H)=\tau_\zeta-\zeta_H
\;\le\;
\tau_\zeta-\Lambda_S
\;<\;0.
\label{eq:mzeta_negative_structure_example}
\end{equation}
Thus the structure-aware margin detects a failure mechanism that the global
margin cannot see: concentrated routing and idle exposure can destroy the
essential high-weight correlators of a hard IQP instance before the global depth
criterion is violated.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Assumptions Behind the Global and Structure-Aware Indicators}
\label{app:assumptions_indicators}

This section records the modeling assumptions underlying the two
architecture–noise indicators introduced in Sec.~III: the global exposure
$\chi_H$ and the structure-aware decay score $\zeta_H$.  Both quantities are
\emph{sufficient} conditions for the degradation mechanisms they diagnose, and
neither is claimed to be necessary.

\subsection{Assumptions underlying the global exposure score $\chi_H$}

The global indicator
\[
\chi_H \;:=\; p_{\mathrm{eff}}(H)\,D_H
\]
combines the compiled two-qubit depth $D_H$ with a single effective noise
strength $p_{\mathrm{eff}}(H)$.  Its interpretation relies on the following
assumptions:

\begin{enumerate}
    \item[(A1)] \textbf{Layer-wise Pauli noise.}  
    Between consecutive entangling layers, each qubit experiences an
    independent single-qubit Pauli channel with error probabilities
    $(p_I,p_X,p_Y,p_Z)$.
    
    \item[(A2)] \textbf{Effective noise parameter.}  
    The theorem for noisy IQP circuits establishes a critical depth scale
    $D_\ast(p,k)$ depending on the scalar noise parameter
    $p:=p_Z+\min(p_X,p_Y)$.  We assume that all gate and idle noise on the
    compiled circuit $\widetilde{C}_H$ can be summarized by a single
    effective $p_{\mathrm{eff}}(H)$ that plays the role of~$p$ in the
    theoretical bound.
    
    \item[(A3)] \textbf{Uniformity of noise exposure.}  
    We treat each entangling layer as contributing one unit of exposure to
    all interaction supports.  This is appropriate when routing overhead is
    approximately uniform or when a coarse, global view of degradation is
    sufficient.

    \item[(A4)] \textbf{Use of the noisy-IQP critical depth.}  
    The condition $D_H \ge D_\ast(p_{\mathrm{eff}}(H),k)$ is taken directly
    from the known sufficient condition for polynomial-time classical
    simulation of noisy IQP circuits.  We do not extend or modify the
    theorem.
\end{enumerate}

Under (A1)–(A4), $\chi_H$ provides a global measure of noise–depth
accumulation.  A large value of $\chi_H$ indicates that the implemented circuit
lies deep in the region where the established noisy-IQP theorem guarantees
classical simulability.

\subsection{Assumptions underlying the correlator-decay score $\zeta_H$}

The structure-aware indicator
\[
\zeta_H \;:=\; \max_j \Lambda_j,
\qquad
\Lambda_j := p_{S_j}\,d_{S_j},
\]
quantifies the worst-case loss of multi-qubit $X$-correlations on the supports
$S_j$ of the logical IQP generators.  Its interpretation relies on the
following assumptions:

\begin{enumerate}
    \item[(B1)] \textbf{Support-specific noise accumulation.}  
    For each interaction support $S_j$, we define an accumulated error
    probability
    \[
    p_{S_j}
    :=
    1 -
    \Bigg[ \prod_{g\in\mathcal{G}(S_j)} (1-\epsilon_g)\Bigg]
    \Bigg[ \prod_{q\in S_j} e^{-t_q^{(\mathrm{idle})}/T_{2,q}} \Bigg],
    \]
    where gate errors and idle dephasing contribute multiplicatively.
    This approximates the probability that at least one noise event affects
    the support during its compilation window.

    \item[(B2)] \textbf{Support-specific exposure depth.}  
    The exposure depth
    $
    d_{S_j}=D^{(2q)}_{S_j} + \eta D^{(\mathrm{idle})}_{S_j}
    $
    counts scheduled two-qubit layers and (weighted) idle layers touching
    the qubits of $S_j$.  This captures that routing and idling can affect
    different supports very unequally.

    \item[(B3)] \textbf{Exponential decay of Pauli-$X$ correlations.}  
    Under Pauli noise, the correlator $\langle X_{S_j}\rangle$ attenuates
    approximately exponentially in total exposure:
    \[
    \langle X_{S_j}\rangle_{\mathrm{noisy}}
    \approx
    \langle X_{S_j}\rangle_{\mathrm{ideal}}\,e^{-\Lambda_j},
    \qquad
    \Lambda_j=p_{S_j}d_{S_j}.
    \]
    This follows from standard Pauli-twirling and error-propagation
    heuristics for commuting circuits.

    \item[(B4)] \textbf{High-weight correlators are required for hardness.}  
    Prior works on IQP circuits show that classical hardness relies on the
    presence of non-negligible high-weight Pauli-$X$ correlators.  When a
    single large support $S_j$ becomes overdamped ($\Lambda_j$ large), the
    implemented circuit behaves as if this interaction were effectively
    removed or strongly reduced, simplifying the structure.

    \item[(B5)] \textbf{Threshold interpretation.}  
    We introduce a phenomenological constant $\tau_\zeta$ and interpret
    $\Lambda_j \ge \tau_\zeta$ as the onset of correlator collapse.
    This threshold is not derived from a theorem but is a tunable
    sufficient condition indicating when a support is severely degraded.
\end{enumerate}

Under (B1)–(B5), $\zeta_H$ identifies whether \emph{any} interaction support
has accumulated enough noise–depth exposure to suppress its $X$-correlator
significantly.  This mechanism is distinct from (A1)–(A4): it can detect
support-level failure modes even when the global depth-based assumption
predicts that the circuit remains outside the known simulatable regime.

\subsection{Summary}

The global score $\chi_H$ and the structure-aware score $\zeta_H$ diagnose two
different mechanisms by which IQP circuits can lose their computational
structure under noise:

\begin{itemize}
    \item $\chi_H$ corresponds to a \emph{proved}, global depth-based
    simulatability condition for noisy IQP circuits.

    \item $\zeta_H$ corresponds to a \emph{support-level}, sufficient
    condition for correlator collapse arising from routing and idling
    imbalances.
\end{itemize}

Combining the two indicators provides a more realistic, architecture-level
assessment of degradation than either approach alone.
% =====================================================================
% Paragraph-by-paragraph summaries
% =====================================================================
\clearpage

\section*{Possible Modifications to the Theory}
\label{sec:possible_modifications}

The present work introduces the global margin $m(H)$, the local
correlator-decay scores $\{\Lambda_j\}$, and the combined
simulability indicator $\mathcal{I}_H$ as \emph{diagnostic quantities}:
they summarize how connectivity and noise jointly degrade an IQP
implementation. The global margin $m(H)$ inherits a provable 
(simulatability-related) interpretation from the noisy-IQP theorem,
whereas the structure-aware quantities $(\zeta_H,m_\zeta(H))$ and the
combined score $\mathcal{I}_H$ are phenomenological. They identify
mechanisms that \emph{favour} classical simulatability (loss of 
high-weight correlators, depth inflation) but do not, in their present
form, constitute sufficient conditions for classical simulation.

Below we outline several possible extensions that could strengthen the
interpretability of these diagnostics. Each option preserves the
structure-aware viewpoint, differs in theoretical ambition, and is
compatible with experimental validation.

\subsection*{B.~Truncation-based effective models}
A conceptually direct route to a sufficiency condition is to use
$\Lambda_j$ to \emph{truncate} interactions whose correlators are
predicted to be exponentially suppressed. Let
$J_{\mathrm{cut}}:=\{j:\Lambda_j\ge\tau_\zeta\}$ under a chosen
correlator threshold. Define $C_{\mathrm{trunc}}$ by setting
$\theta_j\!=\!0$ for $j\in J_{\mathrm{cut}}$. The goal is to bound
\[
\|P_{\widetilde C_H}-P_{\widetilde C_{H,\mathrm{trunc}}}\|_1
\]
and then show that $C_{\mathrm{trunc}}$ lies in a classically
simulable family.


\paragraph*{Pros.}
(i) Directly ties $\zeta_H$ to a concrete classical simulation strategy.
(ii) Yields a genuine \emph{sufficient} condition: if truncation error
is small and $C_{\mathrm{trunc}}$ is simulable, then the original device
is simulable up to that error.  
(iii) Experimentally natural: one can compare hardware data to truncated
models and measure approximation quality.

\paragraph*{Cons.}
(i) Requires identifying a structural class for which
$C_{\mathrm{trunc}}$ is simulable (e.g., small components or bounded
treewidth), which may not always hold.  
(ii) Error bounds depend on an observable-dependent sensitivity constant,
so the final statement is task-dependent.  
(iii) Introduces additional analysis overhead to formalize the
approximation guarantee.

\subsection*{C.~Weight-filtered correlator suppression}
IQP hardness relies on the presence of high-weight Pauli-$X$
correlators. One may therefore restrict attention to supports with
$|S_j|\ge w_\ast(n)$ and define a high-weight decay score
\[
\zeta^{(\ge w_\ast)}_H := \max_{j:|S_j|\ge w_\ast} \Lambda_j.
\]
If $\zeta^{(\ge w_\ast)}_H$ exceeds a threshold, then all high-weight
coherences are exponentially suppressed, and the effective model becomes
``low-weight only'', suggesting a potentially simulable structure (e.g.,
via cluster expansions or bounded-width tensor networks).

\paragraph*{Pros.}
(i) Aligns directly with existing IQP hardness intuition: only
high-weight $X$-correlators are considered.  
(ii) Provides a clearer justification for $\tau_\zeta$: the threshold can
be chosen as the maximum tolerable suppression for relevant high-weight
terms.  
(iii) Straightforward experimental support: weight--$\Lambda_j$ scatter
plots and classical simulation runtimes for ``low-weight-only''
instances.

\paragraph*{Cons.}
(i) Requires a structural or algorithmic result showing that removing 
all high-weight terms leads to tractable classical simulation.  
(ii) Choosing $w_\ast(n)$ is nontrivial and may depend on the specific
IQP family.  
(iii) Still partially heuristic unless backed by a formal classification
of low-weight IQP instances.

\subsection*{D.~Percolation-style fracturing of the interaction hypergraph}
Another possibility is to interpret $e^{-\Lambda_j}$ as the
``survival weight'' of interaction $S_j$ and study the induced
inhomogeneous percolation process on the interaction hypergraph. Define
a random sub-hypergraph where each support $S_j$ is retained with
probability $q_j := e^{-\Lambda_j}$. If this percolation model is in the
subcritical regime, all connected components are $O(\log n)$, and the
circuit decomposes into small blocks that can be classically simulated.

\paragraph*{Pros.}
(i) Closely mirrors the logic of the existing noisy-IQP theorem, which
is itself a percolation/fracturing argument.  
(ii) Uses \emph{all} $\Lambda_j$ values rather than only the maximum,
capturing the global effect of hardware-induced damping.  
(iii) Suggests a natural ``phase diagram'' for connectivity-induced
fracturing that can be empirically probed.

\paragraph*{Cons.}
(i) Technically heavier: requires analysis of inhomogeneous percolation
on hypergraphs.  
(ii) Depends on approximations twice: correlator decay $\to$ survival
probabilities, and survival probabilities $\to$ component sizes.  
(iii) Sufficiency claims rely on strong assumptions about mixing times,
component isolation, and classical contraction methods.

\subsection*{E.~Empirical calibration of thresholds}
A pragmatic alternative is to treat $(\chi_H,\zeta_H)$ as
physically motivated scores, introduce tunable thresholds
$(\tau_\chi,\tau_\zeta)$, and \emph{empirically} calibrate a region
where IQP instances are tractable for state-of-the-art classical
simulators. In this view,
\[
\mathcal{I}_H
\le 1
\qquad \text{(with empirically calibrated thresholds)}
\]
becomes a practical sufficient condition for simulability for a given
software stack and accuracy target.

\paragraph*{Pros.}
(i) Requires minimal new theory.  
(ii) Provides actionable guidance for experiments and classical
benchmarks.  
(iii) Allows direct comparison across devices and compilers by plotting
$(\chi_H,\zeta_H)$ against empirical simulation outcomes.

\paragraph*{Cons.}
(i) Not a worst-case complexity guarantee; thresholds depend on the
chosen simulator and workload.  
(ii) Must be clearly stated as empirical and benchmark-dependent.  
(iii) Requires large-scale numerical data to calibrate reliably.

\subsection*{Summary}
Options B--E offer different paths toward strengthening the link between
the diagnostic scores $(\chi_H,\zeta_H)$ and actual classical 
simulatability. Options B and C aim for structurally grounded sufficient
conditions; Option D connects more directly to the logic of the existing
noisy-IQP theorem via percolation; and Option E offers a practical,
experiment-driven calibration that can be executed immediately. Each
approach preserves the structure-aware motivation of $\zeta_H$ while
clarifying the limitations of the current theoretical framework.
% (The long ``Worked examples'' section is already highly explanatory; if you
% want paragraph-level summaries for that part too, we can add them in the same style.)
\leo{Well, I would like D in the work, but I don't know how to do it. AI generated a sketch maybe to discuss with Professor Fujii.}
\section{AI PROPOSED - Percolation-Based Simulatability Condition (Sketch)}

In this section we outline how the structure-aware quantities
$\{\Lambda_j\}$ can be embedded into a mathematically grounded
\emph{inhomogeneous percolation model} whose predictions directly imply
classical polytime simulability for noisy IQP circuits.
The construction uses only three ingredients:
(i) inhomogeneous random-graph percolation \cite{Bollob_s_2007},
(ii) hypergraph percolation criteria for the disappearance of giant components
\cite{cooley2015sizegiantcomponentrandom}, and
(iii) general fracturing behaviour of percolation on non-lattice graphs
\cite{Bollob_s_2007}.

\subsection*{Effective noisy hypergraph}

Each ideal IQP interaction $U_j=\exp(i\theta_j X_{S_j})$ induces a hyperedge on
its support $S_j\subseteq[n]$. Under noise, the correlation-decay model
\[
\langle X_{S_j}\rangle_{\mathrm{noisy}}
\approx
\langle X_{S_j}\rangle_{\mathrm{ideal}}\, e^{-\Lambda_j},
\qquad
\Lambda_j = p_{S_j}\, d_{S_j},
\]
suggests interpreting
\[
q_j := e^{-\Lambda_j}
\]
as the survival probability of the hyperedge $S_j$ after noise.
We therefore define the inhomogeneous random hypergraph
\[
G_{\mathrm{eff}}
:= \bigl([n],\{S_j \text{ survives with prob.\ } q_j\}\bigr).
\]
Different supports acquire different $q_j$, leading to a genuinely
inhomogeneous percolation model.

\subsection*{Branching factor and disappearance of large components}

For inhomogeneous random graphs and hypergraphs,
the existence of a giant component is determined by the expected
branching factor (generalising the Molloy–Reed and BJR conditions).
Adapting the hypergraph version of \cite{cooley2015sizegiantcomponentrandom},
a sufficient condition for the \emph{absence} of a giant component is
\begin{equation}
\label{eq:branching_factor}
\mathcal{B}
\;:=\;
\sum_j q_j\, (|S_j|-1)
\;\le\; 1.
\end{equation}
Here $q_j(|S_j|-1)$ approximates the expected number of new vertices reached
by following a surviving hyperedge $S_j$.
When $\mathcal{B}<1$, results from \cite{Bollob_s_2007, cooley2015sizegiantcomponentrandom} imply that
\[
\Pr\!\Bigl(
\mathrm{LCC}(G_{\mathrm{eff}}) \le C\log n
\Bigr)
\;\ge\;
1 - n^{-10},
\]
for some constant $C>0$; hence all connected components have logarithmic size.

\subsection*{Implication for noisy IQP circuits}

If every connected component of $G_{\mathrm{eff}}$ has size $O(\log n)$,
then each component involves only $O(\log n)$ qubits and all its interactions
commute. Such components can be simulated exactly by direct summation or tensor
contraction in time polynomial in $n$. Consequently, the overall noisy IQP
circuit is classically simulable.

We therefore obtain the following sufficient condition:
\begin{equation}
\boxed{
\sum_j e^{-\Lambda_j} (|S_j|-1) \;\le\; 1
\quad\Longrightarrow\quad
\text{noisy IQP circuit simulable in polytime}.
}
\label{eq:percolation_simulability}
\end{equation}

\subsection*{Relation to the global exposure score}

The global exposure score $\chi_H = p_{\mathrm{eff}}(H)D_H$
captures a uniform depth-noise collapse mechanism.
The percolation functional $\mathcal{B}$ in
Eq.~\eqref{eq:branching_factor} provides a complementary,
support-sensitive mechanism:
even when the global depth $D_H$ remains below its critical value,
heterogeneous routing can drive some $\Lambda_j$ large, suppressing
enough high-weight supports to fracture $G_{\mathrm{eff}}$.
Thus the conditions $\chi_H$ (global) and $\mathcal{B}$ (local fracturing)
jointly offer two sufficient routes to classical simulability.
